Efficient CSMA using Regional Free Energy Approximations

CSMA (Carrier Sense Multiple Access) algorithms based on Gibbs sampling can achieve throughput optimality if certain parameters called the fugacities are appropriately chosen. However, the problem of computing these fugacities is NP-hard. In this work, we derive estimates of the fugacities by using a framework called the regional free energy approximations. In particular, we derive explicit expressions for approximate fugacities corresponding to any feasible service rate vector. We further prove that our approximate fugacities are exact for the class of chordal graphs. A distinguishing feature of our work is that the regional approximations that we propose are tailored to conflict graphs with small cycles, which is a typical characteristic of wireless networks. Numerical results indicate that the fugacities obtained by the proposed method are quite accurate and significantly outperform the existing Bethe approximation based techniques.

==> Arxiv TMC_journal/abstract.tex <==
CSMA (Carrier Sense Multiple Access) algorithms based on Gibbs sampling can achieve throughput optimality if certain parameters called the fugacities are appropriately chosen. However, the problem of computing these fugacities is NP-hard. In this work, we derive estimates of the fugacities by using a framework called the \emph{regional free energy approximations}. In particular, we derive explicit expressions for approximate fugacities corresponding to any feasible service rate vector. We further prove that our approximate fugacities are exact for the class of \emph{chordal} graphs.  A distinguishing feature of our work is that the regional approximations that we propose are tailored to conflict graphs with small cycles, which is a typical characteristic of wireless networks. Numerical results indicate that the fugacities obtained by the proposed method are quite accurate and significantly outperform the existing Bethe approximation based techniques.


%In this paper, we estimate these attempt rates using the well-known Region-based approximations. The accuracy and complexity of the approximations depend on the choice of regions. Hence, we first propose an approach for an arbitrary collection of regions, and then apply these general results to some ``useful" collection of regions. Specifically, we identify two choices of regions and propose distributed algorithms, which obtain closed form estimates for the attempt rates. We also prove that our algorithm is exact for a class of graphs, called the chordal graphs. Numerical results suggest that the proposed algorithm outperforms the existing Bethe approximation based algorithms for spatial networks.

%The proposed algorithms perform 
%
%we select the regions that significantly improve the
%
%
%the existing approximation algorithms are based on the well-known Bethe approximation framework. This approach is known to incur large error if the network topology consists of many short cycles. Motivated by this fact, we propose two collections of regions that improve the error due to short cycles, and derive the attempt rates in closed form. We also prove that our algorithm is exact for a class of graphs, called the chordal graphs. Numerical results suggest that the proposed algorithm outperforms the existing Bethe approximation based algorithms for spatial networks.
%
%Inspired by the well-known Region-based approximations, we propose two simple distributed algorithms, which obtain closed form estimates for the attempt rates. The accuracy and complexity of the approximations depend on the choice of regions. Hence, we first propose an approach for an arbitrary collection of regions, and then apply these general results to some ``useful" collection of regions. 
%
%The existing approximation algorithms are based on the well-known Bethe approximation framework. This approach is known to incur large error if the network topology consists of many short cycles. Motivated by this fact, we propose two collections of regions that improve the error due to short cycles, and derive the attempt rates in closed form. We also prove that our algorithm is exact for a class of graphs, called the chordal graphs. Numerical results suggest that the proposed algorithm outperforms the existing Bethe approximation based algorithms for spatial networks.


%It is known that CSMA can achieve throughput optimality by sampling feasible schedules from a Gibbs distribution. However, certain parameters of the Gibbs distribution called the fugacities are to estimated to support a given set of service rate requirements. Unfortunately, obtaining these optimal fugacities is an NP-hard problem. Further, the existing algorithms that estimate the fugacities suffer from an impractically slow convergence to the optimal fugacities. To address this issue, we propose an approximation algorithm that gives a closed form solution for the NP-hard problem of computing fugacities. The central idea of our approach is based on the well-known Kikuchi approximation to the underlying Gibbs distribution. We also identify a class of graphs namely chordal graphs for which the proposed algorithm is exact. Numerical results indicate that the proposed method outperforms the existing algorithms for this problem.



==> Arxiv TMC_journal/chordal.tex <==
It is known that the Bethe approximation is exact for tree graphs. In the Kikuchi approximation framework, we have considered larger collection of regions by including the maximal cliques of the graph. Hence, one may expect the accuracy to improve. Indeed, we confirm this intuition by proving that the clique based Kikuchi approximation is exact for a wider class of graphs called the chordal graphs (Trees are a special case of chordal graphs). 


\begin{definition} \emph{(Chordal graph)}
A graph is said to be chordal if all cycles of four or more vertices have a chord. Here, a chord refers to an edge that is not part of the cycle but connects two vertices of the cycle. (See Figure \ref{fig_chordal}, in Section \ref{sec_simulations} for an example of a chordal graph.)
\end{definition}

\begin{theorem} \label{thm_chordal}
If the conflict graph is chordal, the formula proposed in \eqref{eq_main} gives the exact fugacities that correspond to the desired service rates, i.e., if we marginalize the $p(\x)$ \eqref{eq_dist} corresponding to the estimated fugacities $\tilde{v_i}$ \eqref{eq_main}, we obtain the required service rates.
\end{theorem}
\begin{proof}
Proof is provided in Section \ref{proof_chordal}.
\end{proof}

\subsubsection*{Complete graph topology}
Now, we consider the complete graph topology and compute the RAF. Further, since the complete graph is a chordal graph, the RAF are exact.
\begin{cor}
Let the conflict graph be a complete graph. Then, the fugacities that exactly support the desired service rates $\{s_i\}$ are given by
\begin{align*}
\exp(v_i)&= \frac{s_i}{1- \sum_{j \in \N} s_j}, \; \forall i \in \N.
\end{align*}
\end{cor}
\begin{proof}
In a complete graph, the only maximal clique constitutes the whole network. Hence $r = \N$ is the only region in the collection of regions $\Re$. Further, due to \eqref{eq_counting_formula}, the counting number $c_r=1$. Hence, from Theorem \ref{thm_clique}, \ref{thm_chordal} the result follows.
\end{proof}

==> Arxiv TMC_journal/clique_algo.tex <==
We implement the following distributed algorithm at every node to determine maximal cliques that particular node is involved in.


\emph{Algorithm:}We assume that all the nodes are numbered in a centralized fashion and one hop exchange occurs through the network.So, we assume that each node has information about its neighbors and their neighbors i.e the node has information till 2-hop extent.Consider the algorithm at node $i$:
\begin{itemize}
\item Initially consider all the neighbors of $i$ as unmarked.
\item Select an unmarked neighbor $j$ and add it to a new list.
\item Now consider all the neighbors one by one and each time check if this neighbor of $i$ is also a neighbor to all the nodes in the above list.
\item When done with all the neighbors of $i$,we get a list of nodes which belong to a clique.Change the status of all the nodes in this list as marked.
\item If there exists an unmarked neighbor of $i$ go back to step 2 to and proceed by selecting one of unmarked neighbor.Else exit form the algorithm.
\end{itemize}
At the end of this algorithm we will have several lists of nodes,each of which is a clique involving node $i$.The clique involving maximum number of nodes will be maximal clique(s) involving node $i$.


Let us illustrate the algorithm above for node $2$ and node $3$ of conflict graph in \ref{fig_cliq}.Considering node $2$,since we assume that it has knowledge of it's 2-hop network,we have neighbors as $\N_2=\{1,8,7,3\}$ and their neighbors as $\N_1=\{2\}$ , $\N_8=\{2,7\}$, $\N_7=\{8,2,3,5,6\}$ and  $\N_3=\{2,4,5,6,7\}$.Initially let all the neighbors of $2$ be unmarked. Let us select an unmarked node $1$.We add this to a new list resulting in $\{1\}$. Now,checking if other neighbors of $2$ are neighbors of nodes in list.We do not have any such nodes.So,we have one list as $\{1\}$ .So mark $1$ in neighbors list. Now select another unmarked node $8$ and add to new list resulting in $\{8\}$.Checking with other neighbors,we can add $7$ to list because it is in neighbor list and is also a neighbor to node $8$ which makes the list $\{8,7\}$.we mark nodes $8$ and $7$ also. Now considering unmarked nodes,we have node $3$.Add it to new list to get $\{3\}$.Now check for other neighbors and we get that node $7$ can be added to list making it $\{3,7\}$.With this we mark node $3$.Now on checking we see that there are no unmarked neighboring nodes.So we stop and check all the lists obtained which are $\{1\}$,$\{8,7\}$ and $\{3,7\}$.Among these two lists have same maximum length of two because of which both contribute to maximal cliques.So,we have maximal cliques at node $2$ as $\{2,8,7\}$ and $\{2,3,7\}$.
Let us also do this for node $3$.We have neighbors as $\N_3=\{2,4,5,6,7\}$ and their neighbors as $\N_2=\{1,3,7,8\}$ , $\N_4=\{3\}$, $\N_5=\{3,6,7\}$, $\N_6=\{3,5,7\}$ and $\N_7=\{2,3,5,6,8\}$.Initially let all the neighbors of $3$ be unmarked. Let us select an unmarked node $2$.We add this to a new list resulting in $\{2\}$. Now,checking if other neighbors of $2$ are neighbors of nodes in list. We have node $7$ which is added to list. So,we have one list as $\{2,7\}$ .So mark $2$ and $7$ in neighbors list. Now select another unmarked node $4$ and add to new list resulting in $\{4\}$.Checking with other neighbors,we can do not have any nodes to add to list because no neighbor of node $3$ in neighbor of node $4$ which makes the list only $\{4\}$.we mark node $4$ also. Now considering unmarked nodes,we have node $5$.Add it to new list to get $\{5\}$.Now check for other neighbors and we get that node $6$ can be added to list making it $\{5,6\}$.We also notice that node $7$ can also be added to list because node $7$ is neighbor of both node $5$ and $6$ which makes the list $\{5,6,7\}$.With this we mark nodes $5$ and $6$.Now on checking we see that there are no unmarked neighboring nodes.So we stop and check all the lists obtained which are $\{2,7\}$,$\{4\}$ and $\{5,6,7\}$.Among these only one list has maximum length of three because of which it contributes to maximal clique.So,we have maximal clique at node $3$ as $\{3,5,6,7\}$.Visually we can see that the maximal cliques obtained from distributed algorithm are correct.

==> Arxiv TMC_journal/clique_section.tex <==
Let $\Re_0$ be the set of all the maximal cliques in the conflict graph. Let $\Re$ denote the set of regions obtained by including the set of the maximal cliques $\Re_0$, and all the regions that can be obtained by taking all the possible intersections of maximal cliques. Note that this choice of regions ensures that the error-inducing 3-cycles (which are nothing but the cliques of size 3), are included in the collection of the regions $\Re$. Let the counting numbers be obtained by \eqref{eq_counting_formula}.


\subsection{Explicit formula for RAF}
In Theorem \ref{thm_clique}, we derive explicit formula for the RAF.

\begin{theorem} \label{thm_clique}
Let $\Re_0$ be the set of maximal cliques in the conflict graph. Let $\Re$ denote the collection of regions obtained by performing cluster variation method with $\Re_0$ as the initial set of regions. Let the counting numbers be defined by \eqref{eq_counting_formula}. Then, for any given service rate requirements $\{s_i\}$, the Region approximated fugacities are given by
\begin{align}
\exp(\tilde{v}_i)&= s_i  \prod_{\{r \in \Re \; | \; i \in r\}} \Big(1- \sum_{j \in r} s_j\Big)^{-c_r}, \; \; i \in \N. \label{eq_thm_clique}
\end{align}
\end{theorem}
\begin{proof}
Consider the optimization problem \eqref{eq_opt_step1} in Theorem \ref{thm_step1}. Now, we use the fact that any region $r \in \Re$ is a clique, and show that there is a unique set of $\{b_r(\x_r)\}$ that satisfy the feasibility constraints \eqref{eq_normalization} - \eqref{eq_bi_si} of the optimization problem \eqref{eq_opt_step1}. Let $\{b_r(\x_r)\}$ be feasible for \eqref{eq_opt_step1}. Since, every region $r \in \Re$ is a clique, from the definition of local feasibility, no more than one vertex can be simultaneously active in a feasible regional schedule $\x_r \in \I_r$. Hence, the set of local feasible schedules for a clique region $r$ is given by
\begin{align*}
\I_r&=\{\x_r^j\}_{j \in r} \cup \{\bf{0}\}.
\end{align*}
where $\x_r^j$ is the schedule with $x_j=1, x_k=0, \forall k\in r \setminus \{j\}$, and $\bf{0}$ is the schedule with $x_k=0, \forall k \in r$.
%\begin{align}
%b_r(\x_r)=0, \;  \forall \x_r \in \{\x_r \; | \; \sum_{j \in r} x_j > 1\}, \; \forall r \in \Re. \label{eq_infeasible}
%\end{align}
%Using \eqref{eq_infeasible} in t
Then from  the local consistency constraint \eqref{eq_consistency} with $r=\{j\}$ and some $q \supset \{j\}$, we have
\begin{align*}
\sum_{\x_q \in \I_q : x_j=1} b_q(\x_q)&= b_{j}(1), \\
b_q(\x_q^j)&=b_{j}(1).
\end{align*}
Then from \eqref{eq_bi_si}, and the normalization constraint \eqref{eq_normalization}, we conclude that
\begin{align}
b_r(\x_r)=
\begin{cases}
      s_j,  &\text{if } \x_r=\x_r^j,  \\
      1- \sum_{k \in r} s_k,  &\text{if } \x_r=\bf{0}, \label{eq_reg_dist}
\end{cases}
\end{align}
is the only set of regional distributions $\{b_r(\x_r)\}$ that satisfy the feasibility constraints \eqref{eq_consistency} - \eqref{eq_bi_si}. Hence, it is the optimal solution of \eqref{eq_opt_step1}	. Substituting \eqref{eq_reg_dist} in Theorem \ref{thm_step2}, we obtain the RAF as follows:
\begin{align*}
\exp(\tilde{v}_i)&= \prod_{\{r \in \Re \; | \; i \in r\}} \left(\frac{s_i}{1-\sum_{j\in r}s_j}\right)^{c_r}, \; \; \forall i \in \N.
\end{align*}
Further, from \eqref{eq_counting_general}, we have $\sum_{\{r \in \Re | i \in r\}} c_r =1$. Hence, the RAF are given by \eqref{eq_thm_clique}.
\end{proof}

Next, we state a corollary of Theorem \ref{thm_clique} which gives the RAF corresponding to the Bethe approximation framework. This result is known due to \cite{bethe_jshin}, and we present it for the sake of completeness.
\begin{cor} \label{cor_bethe}
The Region approximated fugacities under the Bethe approximation framework are given by
\begin{align}
\exp(\tilde{v}_i)= \frac{s_i (1-s_i)^{|\N_i|-1}}{\prod_{j \in \N_i} (1-s_i-s_j)}, \; \; i \in \N, \label{eq_bethe}
\end{align}
where the set $\N_i$ denotes the neighbours of the vertex $i$ in the conflict graph.
\end{cor}
\begin{proof}
 As discussed earlier, in the Bethe approximation framework, the collection of regions $\Re$ includes only the regions corresponding to the edges and the vertices of the conflict graph, \ie, 
 \begin{align*}
  \Re= \lbrace\{i\}\; |\; i \in V \rbrace \cup \lbrace\{i,j\} \;| \; (i,j) \in E \rbrace.
 \end{align*}
 Since an edge is also a clique of the graph,  the observation \eqref{eq_reg_dist} is valid for the regions in the Bethe approximation framework. Hence, the result \eqref{eq_thm_clique} is applicable for this case.  Now, let us consider the regions of the Bethe approximation, and compute their counting numbers \eqref{eq_counting_formula}. Specifically, for a region $r=\{i, j\}$ corresponding to an edge $(i,j) \in E$ of the conflict graph, the counting number 
 \begin{align*}
c_{\{i,j\}}&= 1- \sum_{\{q \in \Re | \{i,j\} \subset q\}} c_q, \\
&= 1,
 \end{align*}
since a region corresponding to an edge $\{i,j\}$ is not a subset of any another edge or a vertex, \ie, $\{q \in \Re | \{i,j\} \subset q\}$ is an empty set.  

For a region $\{i\}$, corresponding to a vertex, the counting number 
\begin{align*}
c_{i}&= 1- \sum_{\{q \in \Re | \{i\} \subset q\}} c_q, \\
&= 1 - \sum_{j \in \N_i} c_{\{i,j\}},\\
&= 1- |\N_i|.
\end{align*}
Now, substituting these counting numbers in \eqref{eq_thm_clique} gives us the Bethe approximated fugacities \eqref{eq_bethe}.
\end{proof}


\subsection{Distributed Algorithm}
\input{dist_algorithm.tex}

\subsection{Exactness of Clique based approach}
\input{chordal.tex}

==> Arxiv TMC_journal/dist_algorithm.tex <==
\input{figure.tex}
We now propose a distributed algorithm to estimate the fugacities using cluster variation method with cliques as the maximal regions. Each link in the network can independently execute the algorithm once it obtains the a) target service rates of the neighbours, b) the local one-hop neighbourhood topology (See Figures \ref{fig_cliq}, \ref{fig_local_topology} for an example). 


There are mainly two steps in the algorithm at a link $i$. The first step involves computing the maximal cliques, and their intersections in which the link $i$ is part of. The next step is to compute its fugacity by using the formula \eqref{eq_thm_clique}. We introduce some notations before we present the algorithm.

\emph{Notation:} Let $\Re_0^i$ be the collection of maximal cliques of the conflict graph $G(V,E)$ in which the vertex $i$ is part of. For example, if we consider the graph in Figure \ref{fig_cliq},  then $\Re_0^2 =\{\{1,2\}, \{2,8,7\}$, $\{2,3,7\}\}$. Similarly $\Re_0^3= \{\{2,3,7\}, \{3,5,6,7\}, \{3,4\} \}$. Using the information about the local topology, any standard algorithm like \cite{cliques_complexity} can be used for finding this set of maximal cliques $\Re_0^i$. For every maximal clique $r \in \Re_0^i$, let us associate a counting number $c_r=1.$
\noindent\rule[0.5ex]{\linewidth}{0.5pt}
\textbf{Algorithm 1:} Clique based distributed algorithm at link $i$\\
\noindent\rule[0.5ex]{\linewidth}{0.5pt}
\; \; \emph{Input:}  $\Re_0^i$, service rates $\{s_j\}_{j \in \N_i}$; \hspace{0.25cm}
\emph{Output:}  fugacity $\tilde{v}_i$.
\begin{enumerate}
\item Consider a variable $l$ called level, and initialize $l=0$.

\item Obtain $\Re_{l+1}^i$ by intersecting the cliques in level $l$, with the cliques in levels less than or equal to $l$, \ie,
\begin{align*}
\Re_{l+1}^i:= \{q_1 \cap q_2 \;|\;  q_1 \in \Re_{l}^i, q_2 \in \cup_{k \leq l} \Re_{k}^i, \; q_1 \neq q_2\}.
\end{align*}
 If  there are no intersections, \ie, $\Re_{l+1} = \Phi$, go to Step 6; Else continue.

\item From the set $\Re_{l+1}^i$, discard the following:
\begin{itemize}
\item[(i)] Cliques which are already present in a previous level, \ie, discard $r \in \Re_{l+1}^i$ if $r \in \cup_{k \leq l} \Re_{k}^i$.

\item[(ii)] Cliques which are  proper subsets of some other cliques in $\Re_{l+1}^{i}$, \ie, discard $r \in \Re_{l+1}^i$ if there exist any other set $q \in \Re_{l+1}^i$ such that $r \subset q$.
\end{itemize}



\item For each clique $r \in \Re_{l+1}^i$, compute 
\begin{align}
c_r= 1 - \sum_{q \in \S(r)} c_q, \label{eq_counting}
\end{align}
where $\S(r)=\{q \in \cup_{k \leq l}\Re^i_{k}\; | \; r \subset q\}$ is the set of cliques which are super sets of a given set $r$.
\item Increment $l$ by $1$, and go to step 2.

\item Let $\Re^i:= \cup_k \Re_k^i$ denote the collection of all the regions computed above. Then the fugacity is computed as
\begin{align}
\exp(\tilde{v}_i) = s_i \prod_{r \in {\Re^i}} \Big(1- \sum_{j \in r} s_j \Big)^{-c_r}.  \label{eq_main}
\end{align}
\end{enumerate}
\noindent\rule[0.5ex]{\linewidth}{0.5pt}

\emph{Complexity:} The worst case complexity incurred by a link to compute the corresponding maximal cliques $\Re_0^i$ is $O(3^{d/3})$, where $d$ is the the maximum degree of the graph \cite{cliques_complexity}. Hence, for spatial networks, where the degree of the graph does not scale with the network size, our algorithm computes the fugacities with $O(1)$ complexity. 

 \emph{Information exchange:} The information exchange required for our algorithm is very limited, since the algorithm is fully distributed except for obtaining the local topology information and neighbours' service rates.

 \emph{Example:} Let us consider the conflict graph shown in Figure \ref{fig_cliq}, and compute the fugacity for the vertex $2$ using the proposed algorithm. The  local topology, and the set of regions at vertex $2$ are shown in Figures \ref{fig_local_topology}, \ref{fig_reg}. The  set of maximal cliques containing the vertex $2$ is $\Re_0^2 =\{\{1,2\}, \{2,8,7\}$, $\{2,3,7\}\}$. Considering their intersections we get $\Re_1^2=\{\{2,7\}, \{2\}\}$. However, we discard the set $\{2\}$ since it is a proper subset of another region $\{2,7\}$ in the same level. Hence $\Re_1^2= \{\{2,7\}\}$. Now, $\Re_2^2$ is obtained by intersecting $\{2,7\}$ with regions in the previous level $\Re_0^2$. The only new region we obtain is the singleton set $\{2\}$, \ie,  $\Re_2^2=\{\{2\}\}$. 
 
Next, we compute the counting numbers of these regions. As defined earlier, all the maximal cliques $\Re_0^2$ will be given a counting number $1$. Further from \eqref{eq_counting}, it can be easily observed that for the set $r=\{2,7\}$, $c_r=-1$, since it has two super sets namely $q_1=\{2,8,7\}, \;q_2= \{2,3,7\}$  with $c_{q_1}=1, c_{q_2}=1$. Similarly, since every region in $\Re_0^2 \cup \Re_1^2$ is a super set of the region $r=\{2\}$, the counting number of $r=\{2\}$ is $c_r= 1- c_{\{2,7\}} - c_{\{1,2\}} - c_{\{2,8,7\}} - c_{\{2,3,7\}} = -1.$ Hence, the following expression gives the fugacity $\exp(\tilde{v}_2)$:
\begin{align*}
\frac{s_2  (1-s_2-s_7)(1-s_2)}{(1-s_1-s_2) (1-s_2-s_8-s_7) (1-s_2-s_3-s_7)}.
\end{align*}
Next, we prove that the Region approximated fugacities computed using the clique based approach are exact for a class of graphs called the chordal graphs.

==> Arxiv TMC_journal/figure.tex <==
\begin{figure}
\begin{center}
  \hspace{-2mm}
%\begin{minipage}{.25\textwidth}
 % \centering
%  \includegraphics[width=.4\linewidth]{image1}
\begin{tikzpicture}[scale=0.7]

\fill (0.5,0.5)circle(0.06cm);
\fill (3.5,0.5)circle(0.06cm);
\fill (1,2)circle(0.06cm);
\fill (3,2)circle(0.06cm);
\fill (4,2)circle(0.06cm);
\fill (1,1)circle(0.06cm);
\fill (3,1)circle(0.06cm);
\fill (4,1)circle(0.06cm);

\node at (.9,2.2) {\begin{scriptsize}8\end{scriptsize}};
\node at (1.1,.8) {\begin{scriptsize}2\end{scriptsize}};
\node at (3,2.2) {\begin{scriptsize}7\end{scriptsize}};
\node at (2.9,0.8) {\begin{scriptsize}3\end{scriptsize}};
\node at (4.1,2.2) {\begin{scriptsize}6\end{scriptsize}};
\node at (4.1,0.8) {\begin{scriptsize}5\end{scriptsize}};


\draw (1,2)-- (3,2) -- (3,1) -- (1,1) -- (1,2);  % Rectangle



\draw (3,2)-- (4,2) -- (4,1) -- (3,1) -- (3,2); % Square


\draw (1,1) -- (0.5,0.5); % corner line to rect.
\node at (0.35,0.4) {\begin{scriptsize}1\end{scriptsize}};


\draw (3,1) -- (3.5,0.5); % corner line to rect.
\node at (3.65,0.4) {\begin{scriptsize}4\end{scriptsize}};
;

\draw (1,1) -- (3,2); % diag for rect.

\draw (4,1) -- (3,2); % left to right diag for sq

\draw (3,1) -- (4,2); %  right to left diag for sq
\end{tikzpicture}
  \vspace{-2mm}
 \caption{An example of a conflict graph with 8 vertices} 
  \label{fig_cliq}
  \end{center}
  \end{figure}
  
  %Second figure starts..
  \begin{figure}
\begin{center}
  \hspace{-2mm}
%\begin{minipage}{.25\textwidth}
 % \centering
%  \includegraphics[width=.4\linewidth]{image1}
\begin{tikzpicture}[scale=0.7]

\fill (0.5,0.5)circle(0.06cm);
%\fill (3.5,0.5)circle(0.06cm);
\fill (1,2)circle(0.06cm);
\fill (3,2)circle(0.06cm);
%\fill (4,2)circle(0.06cm);
\fill (1,1)circle(0.06cm);
\fill (3,1)circle(0.06cm);
%\fill (4,1)circle(0.06cm);

\node at (.9,2.2) {\begin{scriptsize}8\end{scriptsize}};
\node at (1.1,.8) {\begin{scriptsize}2\end{scriptsize}};
\node at (3,2.2) {\begin{scriptsize}7\end{scriptsize}};
\node at (2.9,0.8) {\begin{scriptsize}3\end{scriptsize}};
%\node at (4.1,2.2) {\begin{scriptsize}6\end{scriptsize}};
%\node at (4.1,0.8) {\begin{scriptsize}5\end{scriptsize}};


\draw (1,2)-- (3,2) -- (3,1) -- (1,1) -- (1,2);  % Rectangle



%\draw (3,2)-- (4,2) -- (4,1) -- (3,1) -- (3,2); % Square


\draw (1,1) -- (0.5,0.5); % corner line to rect.
\node at (0.35,0.4) {\begin{scriptsize}1\end{scriptsize}};


%\draw (3,1) -- (3.5,0.5); % corner line to rect.
%\node at (3.65,0.4) {\begin{scriptsize}4\end{scriptsize}};
;

\draw (1,1) -- (3,2); % diag for rect.

%\draw (4,1) -- (3,2); % left to right diag for sq

%\draw (3,1) -- (4,2); %  right to left diag for sq
\end{tikzpicture}
  \vspace{-2mm}
 \caption{Local neighbourhood topology at vertex $2$ of Figure \ref{fig_cliq}} 
  \label{fig_local_topology}
  \end{center}
  \end{figure}
\begin{figure}
  \centering
  %\includegraphics[width=.4\linewidth]{image1}
  \begin{tikzpicture}[scale=1]

\node at (4,2) {$\Re_0^i$};
\node at (4,1) {$\Re_1^i$};
\node at (4,0.2) {$\Re_2^i$};

\node (rect12) at (5,2) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}1,2\end{scriptsize}};
\node (rect237) at (6,2) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}2,3,7\end{scriptsize}};
\node (rect278) at (7,2) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}2,7,8\end{scriptsize}};
%\node (rect3567) at (8,2) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}3,5,6,7\end{scriptsize}};
%\node (rect34) at (9,2) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}3,4\end{scriptsize}};

\node (rect27) at (6.7,1) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}2,7\end{scriptsize}};
%\node (rect37) at (7.8,1) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}3,7\end{scriptsize}};

%\node (rect7) at (7.2,0.2) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}7\end{scriptsize}};

\node (rect2) at (6.1,0.2) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}2\end{scriptsize}};

%\node (rect3) at (8.4,0.2) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}3\end{scriptsize}};

%\node[state] (A) {G};
%  \node[state] (B) [right of=A] {B};


  \path (rect237) edge (rect27);
    \path (rect278) edge (rect27);
%     \path (rect237) edge (rect37);
%      \path (rect3567) edge (rect37);
 %      \path (rect27) edge (rect7);
%        \path (rect37) edge (rect7);
        \path (rect12) edge (rect2);
        \path (rect27) edge (rect2);
%         \path (rect37) edge (rect3);
%        \path (rect34) edge (rect3);
 % \path (B) -- (A);

\end{tikzpicture}
\captionof{figure}{Pictorial representation of the intersections of the cliques at vertex $i=2$.}
  \label{fig_reg}
\end{figure}





%\begin{figure}
%  \centering
%  %\includegraphics[width=.4\linewidth]{image1}
%  \begin{tikzpicture}[scale=1]
%
%
%
%\node (rect12) at (5,2) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}1,2\end{scriptsize}};
%\node (rect237) at (6,2) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}2,3,7\end{scriptsize}};
%\node (rect278) at (7,2) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}2,7,8\end{scriptsize}};
%\node (rect3567) at (8,2) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}3,5,6,7\end{scriptsize}};
%\node (rect34) at (9,2) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}3,4\end{scriptsize}};
%
%\node (rect27) at (6.7,1) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}2,7\end{scriptsize}};
%\node (rect37) at (7.8,1) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}3,7\end{scriptsize}};
%
%\node (rect7) at (7.2,0.2) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}7\end{scriptsize}};
%
%\node (rect2) at (5.8,0.2) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}2\end{scriptsize}};
%
%\node (rect3) at (8.4,0.2) [draw,minimum width=.25cm,minimum height=.25cm] {\begin{scriptsize}3\end{scriptsize}};
%
%%\node[state] (A) {G};
%%  \node[state] (B) [right of=A] {B};
%
%
%  \path (rect237) edge (rect27);
%    \path (rect278) edge (rect27);
%     \path (rect237) edge (rect37);
%      \path (rect3567) edge (rect37);
%       \path (rect27) edge (rect7);
%        \path (rect37) edge (rect7);
%        \path (rect12) edge (rect2);
%        \path (rect27) edge (rect2);
%         \path (rect37) edge (rect3);
%        \path (rect34) edge (rect3);
% % \path (B) -- (A);
%
%
%\end{tikzpicture}
%\captionof{figure}{Region graph}
%  \label{fig_reg}
%\end{figure}





==> Arxiv TMC_journal/fug_comp.tex <==
Now, we could use results obtained from optimizing Kikuchi free energy function and locally compute fugacities at each node. 
Consider a node $i$. Till this point, we have information about all the regions at various levels of which node $i$ is part of. We also have computed $c_R$ for every region. We can now compute approximate global fugacities locally at this node using the formula as follows:
\noindent\rule[0.5ex]{\linewidth}{0.5pt}
\textbf{Fugacity at node $i$}\\
\noindent\rule[0.5ex]{\linewidth}{0.5pt}
\; \; \emph{Input:} $\{R,c_R\}$; \hspace{0.25cm}
\emph{Output:} $\lt_i$.
The optimal fugacity at node $i$ is given by as
\begin{align}
\lt_i =  \prod_{r \in {R}} \left(\frac{b_r(i=1)}{b_r(i=0)}\right)^{c_r} .  \label{eqn_imp}
\end{align}
where for every region $r$ from ${R}$, 
we have $b_r(i=1)$ as joint probability of region where all the nodes of region are in off/0 state while node $i$ is active. Since the region is clique ,we have
\begin{align}
b_r(i=1) = b_i . \label{side_1}
\end{align}
where $b_i$ is service rate of node $i$.
And we have $b_r(i=0)$ as joint probability of region where all the nodes of region are in off/0 state. Since the region is clique ,we have
\begin{align}
b_r(i=0) = 1 - \sum_{k \in r} b_k . \label{side_2}
\end{align}
where for every node $k$ belonging to the region $r$ we have $b_k$ as service rate of node $k$.
While $c_r$ is the $c_R$ value of region $r$.
\noindent\rule[0.5ex]{\linewidth}{0.5pt}

==> Arxiv TMC_journal/fug_proof.tex <==
In this section, we state our main theorem which explains the connection between our distributed algorithm for the fugacities, and the Kikuchi approximation. Recall that $\Re^i$ is the set of cliques computed in the distributed algorithm at link $i$. Then, it can be easily verified that the set of regions given by $\Re:= \cup_{i=1}^N \Re^i$, with $\{c_r\}$ computed in \eqref{eq_counting}, constitute a valid collection of Kikuchi regions\footnote{In fact, the regions computed in this paper are inspired by the cluster variation method \cite{yedidia}, which is a standard algorithm to generate valid regions.}, and counting numbers. 
%Further, the set of local consistency conditions can be captured using a region graph with the cliques in $\Re$ as its vertices. For example, Figure \ref{fig_reg} shows the region graph corresponding to the conflict graph considered in Figure \ref{fig_cliq}.

\begin{comment}
\begin{figure}
\centering
\includegraphics[scale=0.45]{regions.png} 
%\includegraphics[scale=0.31]{random_graph_new.eps} 
\caption{Region graph for conflict graph shown in Figure \ref{fig_cliq}}
\label{fig_reg}
\end{figure}
\end{comment}

The non trivial step of our algorithm is the formula \eqref{eq_main} proposed for the fugacities. The following theorem justifies the proposed formula. If CSMA algorithm employs the set of fugacities $\{\tilde{v}_i\}_{i=1}^N$ estimated in \eqref{eq_main}, then the service rates obtained by the CSMA, are close to the desired service rates. This is because, the desired service rates correspond to stationary point of the KFE defined by $\{\tilde{v}_i\}_{i=1}^N$ as stated below.
\begin{theorem} \label{thm_main}
Let $\tilde{\v}$ be a set of fugacities that define the Kikuchi free energy $F_K(\{b_r\}; \tilde{\v})$. A locally consistent set of pseudo marginals $\{b_r\}$ will be a stationary point of the KFE if and only if $\sum_{j \in r} b_j(1) < 1, \forall r \in \Re$, and
%\begin{align*}
%\exp(\vt_i)= \prod_{r \in \Re^i}\left(\frac{b_i(x_i=1)}{1-\sum_{j \in {r}}b_j(x_j=1)}\right)^{c_r}, \; \forall i
%\end{align*}
\begin{align}
\exp(\vt_i)= b_i(1) \prod_{r \in \Re^i}\Big(1-\sum_{j \in {r}}b_j(1)\Big)^{-c_r}, \; \forall i, \label{eq_thm}
\end{align}
where $b_i(x_i), b_j(x_j)$ are the regional distributions corresponding to the singleton region sets $\{i\}, \{j\}$ respectively.
\end{theorem}
\begin{proof}
Recall that a schedule $\x=\{x_i\}$ is feasible iff no two adjacent links of the conflict graph transmit simultaneously. Since all our regions are cliques of the conflict graph, for any feasible distribution that is locally consistent, we have  
\begin{align}
b_r(x_r)=
\begin{cases}
      b_j(1),  &\text{if } x_j=1, x_k=0, \forall k \in r\setminus \{j\},  \\
      1- \sum_{j \in r} b_j(1),  &\text{if } x_j=0, \forall j \in r, \\
      0,  &\text{otherwise}. \label{eq_reg_dist}
\end{cases}
\end{align}
An interesting implication of the above observation is, the KFE $F_k(\{b_r\}; \tilde{\v})$ in \eqref{eq_kfe}, which is in general a function of all the pseudo marginals, can now be expressed as a function of the singleton marginals alone. Specifically, the average energy is
\begin{align*}
U_K(\{b_r\}; \tilde{\v})&= - \sum_{r \in {\Re}} c_r \E_{b_r}\Big[\sum_{j \in r} \vt_j x_j\Big], \\
&= - \sum_{r \in {\Re}} c_r \Big( \sum_{j \in r} \vt_j b_j(1)  \Big), \\
&= -\sum_{j=1}^N \Big(\sum_{\{r \;|\; j \in r\}} c_r \Big) \vt_j b_j(1) = -\sum_{j=1}^N \vt_j b_j(1).
\end{align*}
Similarly, the term corresponding to a region $r$ in the Kikuchi entropy $H_K(\{b_r\})$ defined in \eqref{eq_k_ent} can be expressed as
\begin{align*}
&\sum_{x_r}b_r(x_r)\log b_r(x_r) \\
&= \Big(1-\sum_{j \in {r}}b_j(1)\Big)\log\Big(1-\sum_{j \in {r}} b_j(1)\Big) + \sum_{j \in {r}}b_j(1) \log b_j(1).
\end{align*}
Using this expression, the gradient of the Kikuchi free energy $F_K(\{b_j(1)\}; \tilde{\v})$ can be computed as
\begin{align*}
\frac{\partial F_K}{\partial b_i(1)} 
&= -\vt_i + \sum_{\{r | i \in r\}}c_r\Big(\log b_i(1) - \log\big(1-\sum_{j\in {r}}b_j(1)\big)\Big).
\end{align*}
By using the fact that $\sum_{\{r \in \Re | i \in r\}} c_r =1$, and setting the gradient to zero, the proof is complete.
\end{proof}

Next, we state a corollary of Theorem \ref{thm_main} which derives the fugacities that correspond to the Bethe approximation framework used in \cite{bethe_jshin}. Specifically, if the collection of regions $\Re$ is formed using only the edges and the vertices of the conflict graph, it results in the Bethe approximation framework.
\begin{cor}
For a given set of required service rates, the estimate of the fugacities $\{v_i^B\}$ obtained using the Bethe approximation framework is given by
\begin{align*}
\exp(v_i^B)= \frac{s_i (1-s_i)^{d_i-1}}{\prod_{j \in \N_i} (1-s_i-s_j)}, \; \forall i,
\end{align*}
where the set $\N_i$ denotes the neighbours of the vertex $i$ in the conflict graph, and the $d_i$ denotes the degree.
\end{cor}
\begin{proof}
The proof follows by observing a set of valid counting numbers for the regions. Specifically, the counting number of the regions corresponding to each edge in the conflict graph can be set to $1$, and the counting number of a region corresponding to a vertex can be set to $1-d_i$. Then using \eqref{eq_thm}, the proof is completed.
\end{proof}


%While it is easy to argue that the claim is true, it also follows from the fact that our distributed algorithm for computing the regions is inspired by a standard approach called cluster variation method \cite{book_martin} that is generally used to generate valid Kikuchi regions.


%\begin{theorem} \label{thm_kikuchi_free}
%Let $\{\vt_i\}_{i=1}^N$ be the fugacities estimated using \eqref{eq_main}. Then we get that the given service rates $\{s_i\}_{i=1}^N$ are obtained as stationary point for optimizing corresponding free energy function.
%\end{theorem}
%\begin{proof}
%
%Now,we consider the second part of kikuchi free energy. For every region we compute the term $\sum_{x_r}b_r(x_r)\log b_r(x_r)$. Since every region in kikuchi approximation is of clique form we have a generalized form.
%We have, 
%\begin{align}
%\sum_{x_r}b_r(x_r)\log b_r(x_r) = \sum_{i \in {r}}b_i\log(b_i) + (1-\sum_{i \in {r}}b_i)\log(1-\sum_{i \in {r}}b_i)	\label{eqn_proof_right}
%\end{align}
%When we consider the whole kikuchi free energy function we will have term from \eqref{egn_proof_left} and for each region we have term from \eqref{eqn_proof_right}. To optimize the free energy we partially differentiate free energy with service rate of each node as variable and set differentials to $0$.
%Consider a node $i$. When we partially differentiate free energy with respect to service rate $b_i$ of node $i$, term from \eqref{egn_proof_left} gives
%\begin{align}
%\frac{\partial}{\partial b_i} \Big[ -\sum_{i \in {V}}b_im_i  \Big] = -m_i \label{eqn_final_left}
%\end{align}
%Now, when term from \eqref{eqn_proof_right} for region $r$ is partially differentiated with $b_i$, it gives $0$ if region does not contain node $i$. If region contains node $i$, then we get two terms containing $b_i$ which get affected by differentiation.
%We Know,
%\begin{align}
%\frac{\partial}{\partial b_i} \Big[ x\log(x) \Big] = 1+\log(x) \label{eqn_diff_log1}
%\end{align}
%\begin{align}
%\frac{\partial}{\partial b_i} \Big[ (1-x
%)\log(1-x) \Big] = -1-\log(1-x) \label{eqn_diff_log2}
%\end{align}
%So,from \eqref{eqn_diff_log1} and \eqref{eqn_diff_log2} we get 2 terms from each region containing node $i$ which are $\log(b_i)$ and $-\log(1-\sum_{i \in {r}}b_i)$ which get multiplied by $c_r$.
%On a whole we get,
%\begin{align}
%-m_i+ \sum_{r \in {R}}c_r\left(\log(b_i)-\log(1-\sum_{i \in {r}}b_i)\right)=0
%\end{align}
%which can be written as
%\begin{align}
%-m_i+ \sum_{r \in {R}}\log\left(\frac{b_i}{1-\sum_{i \in {r}}b_i}\right)^{c_r}=0
%\end{align}
%If $\lt_i$ is introduced,we get
%\begin{align}
%\lt_i = \prod_{r \in {R}}\left(\frac{b_i}{1-\sum_{i \in {r}}b_i}\right)^{c_r}
%\end{align}
%which is same as
%\begin{align}
%\lt_i =  \prod_{r \in {R}} \left(\frac{b_r(i=1)}{b_r(i=0)}\right)^{c_r}
%\label{eqn_proof_fin}
%\end{align}
%This way we get many equations when free energy is partially differentiated with respect to all the nodes of network.These equations turn out to be the same approximate expressions used to compute fugacities $\{\lt\}_{i=1}^N$.
%Thus we prove that such approximately computed fugacities optimize kikuchi free energy for given set of service rates $\{s_i\}_{i=1}^N$.
%\end{proof}

==> Arxiv TMC_journal/intro_kikuchi.tex <==
\IEEEPARstart{L}{ink} scheduling algorithms based on CSMA have received renewed attention, since they were recently proven to be throughput optimal~\cite{libin,qcsma,sinr_mimo}, in addition to being amenable to distributed implementation. The central idea lies in sampling the feasible schedules from a product form distribution, using a reversible Markov chain called the Gibbs sampler~\cite[Chapter 7]{bremaud}. In order to support a feasible service rate vector, certain parameters of the Gibbs distribution called the fugacities are to be appropriately chosen. However, the problem of computing the fugacities for a desired service rate vector is NP-hard~\cite{libin}. An  iterative algorithm based on stochastic approximation is proposed in~\cite{libin}, which asymptotically converges to the exact fugacities. However, the convergence time of this algorithm scales exponentially with the size of the network~\cite{fast_mixing}. Hence, it is not amenable to practical implementation in large networks.

In this work, we derive estimates of the fugacities by using \emph{regional free energy approximations}~\cite{yedidia} for the underlying Gibbs distribution. In particular, we derive explicit expressions for approximate fugacities corresponding to any feasible service rate vector. Since, the proposed method does not involve any iterative procedures, it does not suffer from convergence issues. A distinguishing feature of our work is that the regional approximations that we propose are tailored to conflict graphs with small cycles, which is a typical characteristic of wireless networks. We also prove that our approximate fugacities are exact for the class of \emph{chordal} graphs. 

%Further, numerical results indicate that the fugacities obtained by the proposed method are quite accurate and significantly outperform the existing approximation techniques~\cite{bethe_jshin}.

%This work proposes efficient closed form approximations for this problem based on Region approximations.

%Main contributions:
%1. We derive explicit expressions for the fugacitites corresponding to any feasible service rate vector using regional free energy approximations. Since, the proposed method does not involve any iterative procedures, it does not suffer from convergence issues.
%
%2. A distinguishing feature of our work is that the regional approximations we propose are tailed to conflict graphs with small cycles which is typical characteristic of wireless networks.
%
%3. We also show that our estimated fugacities are exact for the class of \emph{chordal} graphs \cite{chordal}.
%
%4. Numerical results indicate that the fugacities obtained by the proposed method are quite accurate and significantly outperform existing approximations.
%
%
%
%We approximate the GFE using certain locally consistent approximations called the regional free energy approximations. 
%1) Closed form expressions (No gradient descent)
%2) Tailored to spatial networks


%While the use of regional free energy approximations to approximate the Gibbs distribution is a well known technique, the significance of our contribution lies in deriving explicit expressions for the approximate fugacities. 

%the accuracy of the Region-based approximation crucially depends on the choice of the regions. As the collection of regions becomes larger, the accuracy improves. However, for arbitrary choices of regions, the computation of RAF may not be amenable to a distributed implementation. Hence, the major challenge in using this Region-based approximation framework for an algorithm like CSMA, is in choosing the regions that are as large as possible, while retaining the property of distributed implementation. 
%This regional free energy approximation framework results in different approximations for different choices of regions in the conflict graph.

In the regional approximation framework, the vertices of the conflict graph are divided into smaller subsets called regions, and the Gibbs distribution is approximated  using certain locally consistent distributions over these regions. Specifically, the Gibbs free energy, which is a function of the Gibbs distribution, is approximated using a function of these local distributions called the Regional Free Energy (RFE). 

In this paper, we propose a general framework to find the approximate fugacities for any given conflict graph, and an arbitrary collection of regions. Our framework involves solving a regional entropy maximization problem, which is then used to find the approximate fugacities. While the approach we propose is applicable to any arbitrary choice of regions, the regional entropy maximization problem may not be amenable to a distributed solution. Furthermore, the accuracy of the approximation depends strongly on the choice of regions. Therefore a major challenge in obtaining a practically useful algorithm based on the regional approximation framework lies in judiciously choosing regions to ensure that the resulting CSMA algorithm is both accurate and amenable to distributed implementation. 

Spatial network models like the random geometric graphs \cite{baccelli_book} that are typically used to model the wireless networks contain many short cycles. For such topologies, traditional approaches based on Belief propagation and the Bethe free energy approximation \cite{bethe_jshin} tend to lead to inaccurate approximations of the fugacities, since they are tailored to tree-like structures. This motivates us to choose regions that explicitly include small cycles. In particular, we consider two choices of regions namely: i) \emph{Clique based regions}, which improves the error due to 3-cycles, and ii) \emph{Clique plus 4-cycle based regions}, which improves the error due to both 3, 4-cycles. 

Under these choice of regions, we derive a simple closed form solution for the regional maximum entropy problem. In particular, we first prove that the regional maximum entropy problem decouples into local entropy maximization problems over each region. Then, we derive closed form solutions for these local entropy maximization problems. Thus, the approximate fugacities can be explicitly computed without solving any optimization problems. We further prove that these approximate fugacities are exact for the class of chordal graphs.
%The existing Bethe approximation algorithms are not accurate for network topologies that contain many short cycles. In particular, the cycles of sizes 3, 4 contribute for most of the error.  Unfortunately, 

%spatial network models like the Random geometric graphs \cite{baccelli_book} that are typically used to model the wireless networks contain many short cycles. Hence, it is very important to improve the error due to the 3-cycles and 4-cycles. To that end, we propose two choices of regions namely: i) \emph{Clique based regions}, which improves the error due to 3-cycles, and ii) \emph{Clique plus 4-cycle based regions}, which improves the error due to both 3, 4-cycles. Under these choice of regions, we prove that the two step procedure proposed for computing the RAF boils down to a simple closed form solution. In particular, we first prove that the approximate maximum entropy problem decouples into local entropy maximization problems at each region. Then, we derive closed form solutions for these local entropy maximization problems. Hence, effectively the RAF fugacities can be explicitly computed without solving any optimization problems. 

%Under these choice of regions, we first prove that the two step procedure proposed for computing the RAF boils down to a simple closed form solution. 

% \emph{Clique plus 4-cycle based regions:} Under these choices of regions, we first prove that the approximate maximum entropy problem decouples into local entropy maximization problems at each region. We further derive closed form solution for the local entropy maximization problem. Hence, effectively the RAF fugacities can be explicitly computed without solving any optimization problems. 

We evaluate the performance of our algorithms over spatial networks modelled using geometric random graphs. Numerical results indicate that the fugacities obtained by the proposed method are quite accurate, and significantly outperform the existing Bethe approximation based techniques~\cite{bethe_jshin}.  

\subsection*{Related work}
In the literature, some special cases of the regional approximation framework are used to estimate the fugacities. Bethe approximation~\cite{bethe_jshin, allerton_bethe}  is one such special case.  The Bethe approximation is accurate when the underlying topology is tree-like. However, for spatial networks, which inherently contain many short cycles, the Bethe approximation~\cite{yedidia} may not be the right choice. An iterative approximation algorithm based on Inverse Generalized Belief Propagation (I-GBP) is proposed in \cite{bp_csma}. While the I-GBP considerably improves the performance in the presence of short loops, it suffers from convergence issues. In particular, it is not always guaranteed to converge, and hence not very reliable \cite{bethe_jshin}. In \cite{chordal}, closed form expressions for the fugacities are computed for chordal graphs using a technique called the Junction tree based decomposition \cite{book_martin}. 

%As our algorithms are also exact for chordal graphs, our work establishes an interesting connection that the Region-based approximation framework coincides with the junction tree based approach for chordal graphs.


The rest of the paper is organised as follows. In Section \ref{sec_model}, we introduce the system model. In Section \ref{sec_rfe}, we review the concept of Regional free energy approximation. In Section \ref{sec_inverse}, we propose a unified framework to compute the approximate fugacities under arbitrary choice of regions.  In Section \ref{sec_choice}, we investigate the  accuracy and complexity of different choices of regions. In Section \ref{sec_clique}, we present our results for clique-based regions. In Section \ref{sec_four_cycles}, we derive the results corresponding to clique plus 4-cycle based regions. In Section \ref{sec_simulations}, we present our numerical results.

%\noindent \emph{Comments on complexity and accuracy:}
%In our clique based approach, each node in the network should obtain its one-hop neighbourhood topology to compute the cliques regions. This incurs a complexity of $O(2^{|\N_i|})$, where $\N_i$ is the neighbourhood of node $i$. We would like to emphasise that this complexity depends only the neighbourhood size, and is significantly better than the stochastic approximation based algorithms whose complexity is exponential in the size of the total network size.
%
%In our Clique plus 4-cycle based algorithm, a node should obtain two-hop neighbourhood information, to compute the 4-cycle regions. We remark that the existing I-GBP \cite{bp_csma} based algorithms incur similar complexity since the I-GBP also requires a node to obtain two hop neighbourhood information. However, the I-GBP algorithm suffers from convergence issues, which is not an issue in our algorithm.

%Minimizing the RFE corresponding to a given fugacities (Gibbs distribution) gives the service rates (as the optimal regional distributions corresponding to a singleton region). However, in this paper we are interested in finding the fugacities for a given service rate, not the other way around. In general, for arbitrary choice of regions, there is no simple solution to estimate the fugacities. Hence, we have the following challenges to deal with:
%
%\begin{itemize}
%\item Does there exist a unified framework to estimate the fugacities using the concept of regional free approximations?
%
%\item Is that framework amenable to distributed implementation?
%
%\item What choice of regions lead to accurate results for typical wireless topologies?
%\end{itemize}
%
%
%This approach involves solving an approximate entropy maximization problem, which is possibly a non convex problem. The solution of this problem is then used to find the approximate fugacities. 
%
%While this approach is applicable for arbitrary choice of regions, the approximate entropy maximization problem may not be amenable to a distributed solution. Hence, the major challenge in using this framework for an algorithm like CSMA, is in choosing the regions that result in accurate approximations, while retaining the property of distributed implementation. Spatial network models like the Random geometric graphs \cite{baccelli_book} that are typically used to model the wireless networks contain many short cycles. For such topologies, traditional approaches based on Belief propagation and the Bethe free energy approximation \cite{bethe_jshin} tend to lead to inaccurate approximations of the fugacities, since they are tailored to tree-like structures. This motivates us to propose regional free energy approximations, wherein the choice of regions is tailored to typical topologies induced by wireless interference.






==> Arxiv TMC_journal/inverse_problem.tex <==
%As discussed in Section \ref{sec_rfe}, the Region-based approximation framework is useful in estimating the marginal distributions $\{b^*_r\}$ of a given product form distribution $p(\x)$ (specified by the fugacities $\{v_i\}$ as given in \eqref{eq_dist}) . In particular, the singleton marginals $\{b^*_i(1)\}$ correspond to the estimates of service rates $\{s_i\}$. Hence, this approximation framework is generally useful to estimate the service rates for given fugacities.

As discussed in Section \ref{sec_rfe}, the Regional approximation framework is generally used to estimate the service rates for given fugacities.
%Hence in the context of CSMA, Region-based approximation can be considered as a black box which takes the fugacities and returns the corresponding service rates (See Figure \ref{fig_block}). 
%The problem of estimating the service rates for a given fugacities will be referred to as the \emph{forward problem}. Next, we introduce the following shorthand notation for this forward problem.
%We write $\{v_i\}\xrightarrow[]{\Re} \{s_i\}$ to mean the following: Consider the RFE $F_{\Re}(\{b_r\}; \v)$ corresponding to the fugacities $\{v_i\}$. Then there is a stationary point $\{b_r^*\}$ of the RFE $F_{\Re}(\{b_r\}; \v)$ such that its corresponding singleton marginals are equal to the service rates $\{s_i\}$, \ie, $b_i^*(x_i=1)=s_i, \; \; \; i=1\dots N$.
However, in this work, we use the Regional approximation not to estimate the service rates, but to design an algorithm to estimate the fugacities for given service rate requirements. To that end, we introduce the notion of Region approximated fugacities (RAF).
\begin{definition} (Region approximated fugacities)
Consider the RFE $F_{\Re}(\{b_r\}; \v)$ corresponding to some fugacities $\{v_i\}$. If there is a stationary point $\{b_r^*\}$ of the RFE $F_{\Re}(\{b_r\}; \v)$, such that its corresponding singleton marginals are equal to the desired service rates $\{s_i\}$, \ie, $b_i^*(x_i=1)=s_i, \; \; \; i=1\dots N$, then the fugacities $\{v_i\}$ are said to be Region approximated fugacities for the given service rates $\{s_i\}$.
\end{definition}


\begin{comment}

\begin{figure}[h]
\centering
\begin{tikzpicture}
\draw (0-1, 0) -- (2-1,0);
\draw (0-1, 1.5) -- (0-1,0);
\draw (0-1, 1.5) -- (2-1,1.5);
\draw (2-1, 1.5) -- (2-1,0);
\draw [-to,shorten >=-1pt,gray,ultra thick] (-0.7-1, 0.75) -- (-0.1-1,0.75);
\draw [-to,shorten >=-1pt,gray,ultra thick] (2.05-1, 0.75) -- (2.75-1,0.75);
\node at (-1.5-1,0.75+0.2) {fugacities};
\node at (-1.5-1, 0.4+0.15) {$\{v_i\}_{i=1}^N$};
\node at (1-1,1.2) {Compute};
\node at (1-1,0.9) {a stationary};
\node at (1-1, 0.6) {point};
\node at (1-1, 0.3) {of RFE};
\node at (1-1, -0.35) {\emph{Estimating service rates for given fugacities}};
\node at (3.6-1,0.4+0.15) {$\{b^*_r\}$};
\node at (3.6-1, 0.75+0.2) {marginals};

\draw (-1.5+2.2, -2.5) -- (-0.5+2.2, -2.5);
\draw (-1.5+2.2, -1) -- (-0.5+2.2,-1);
\draw (-1.5+2.2, -2.5) -- (-1.5+2.2, -1);
\draw (-0.5+2.2, -2.5) -- (-0.5+2.2,-1);
\node at (-3+3.1,0.75-2.5+0.3) {$\{b^*_r\}$};
%\node at (-2,0.75-2.5+0.3) {$\bv^*$};
%\node at (-3+3.1,-2.9) {Inverse problem};

\draw (-1.5, -2.5) -- (-0.5, -2.5);
\draw (-1.5, -1) -- (-0.5,-1);
\draw (-1.5, -2.5) -- (-1.5, -1);
\draw (-0.5, -2.5) -- (-0.5,-1);
\node at (-1, -1.75) {Step1};
%\node at (-3+1,0.75-2.5+0.3) {$\bv^*$};
\draw [-to,shorten >=-1pt,gray,ultra thick] (-2.4, 0.75-2.5) -- (-1.6,0.75-2.5);
\draw [-to,shorten >=-1pt,gray,ultra thick] (-0.4, 0.75-2.5) -- (0.5,0.75-2.5);
\draw [-to,shorten >=-1pt,gray,ultra thick] (1.55+0.2, 0.75-2.5) -- (2.2,0.75-2.5);
\node at (-3,0.75-2.5+0.3) {service};
\node at (-3,0.75-2.5) {rates};
\node at (-3+0.1,0.5-2.7) {$\{s_i\}_{i=1}^N$};
%\node at (1+0.2,1.1-2.75-0.3) {(IBO)};
\node at (-3+3.1,-2.9) {\emph{Estimating the fugacities for given service rates}};
\node at (1+0.2,-1.75) {Step2};
%\node at (1, 0.6-3) {optimization};
\node at (3, 0.75-2.5+0.2) {fugacities};
\node at (3, 0.3-2.5+0.2) {$\{v_i\}_{i=1}^N$};
\end{tikzpicture}
\caption{Block diagram for the forward and the reverse problems}
\label{fig_block}
\end{figure}
\end{comment}
We propose a two step approach to compute Region approximated fugacities.
\begin{enumerate}
\item Find a set of locally consistent regional distributions $\{b_r\}$ with the following two properties:
\begin{enumerate}
\item[(P1.)] The marginals corresponding to the singleton regions are equal to the the desired service rates, \ie, $b_i(x_i=1)=s_i, \; \; \; i=1\dots N.$
\item[(P2.)] There exists a set of fugacities $\{v_i\}_{i=1}^N$ for which, the set of regional distributions $\{b_r\}$ is a stationary point of the corresponding RFE $F_{\Re}(\{b_r\}; \v).$
\end{enumerate}
\item Explicitly find those fugacities $\{v_i\}_{i=1}^N$ that satisfy P2.
\end{enumerate}


In Theorem \ref{thm_step1}, we state that obtaining a set of regional distributions $\{b_r\}$ with the properties P1 and P2, boils down to constrained maximization of the regional entropy.
 \begin{theorem} \label{thm_step1}
 Let $\{b_r^*\}$ be some local optimizer of the optimization problem \eqref{eq_opt_step1}. Then $\{b_r^*\}$ satisfies the properties P1 and P2.
 \begin{align}
 &\arg \max_{\{b_r\}}  \sum_{r \in \Re} c_r H_r(b_r), \; \; \; \text{subject to} \label{eq_opt_step1}\\
b_r(\x_r)& \geq 0, \; \x_r \in \I_r; \; \sum_{\x_r \in \I_r} b_r(\x_r) =1, \;r \in \Re, \label{eq_normalization} \\
\sum_{\x_q \setminus \x_{r}} b_q (\x_q) &= b_r(\x_r), \; \; \x_r \in \I_r, \text{ and } r, q \in \Re \text{ s.t. } r \subset q, \label{eq_consistency} \\
% b_r(\x_r)&=0, \; \; \; \x_r \notin \I_r, r \in \Re,  \label{eq_hard} \\
 b_i(1)&=s_i, \; \; \; i=1\dots N. \label{eq_bi_si}
\end{align}  
\end{theorem}
\begin{proof}
The property (P1) trivially follows from \eqref{eq_bi_si}. We provide the proof for property (P2) in Section \ref{proof_thm_step1}.
\end{proof}


Next, in Theorem \ref{thm_step2}, we propose a formula to compute the Region approximated fugacities.
\begin{theorem} \label{thm_step2}
 Let $\{b_r^*\}$, be a local optimizer of \eqref{eq_opt_step1}.  Then the fugacities
\begin{align}
\exp(\tilde{v}_i)&= \prod_{\{r \in \Re \; | \; i \in r\}} \left(\frac{b_r^*(\x_r^i)}{b_r^*(\bf{0})}\right)^{c_r}, \; \; \forall i \in \N, \label{eq_lf_gf}
\end{align}
are Region approximated fugacities for the desired service rates $\{s_i\}$. Here $\x_r^i$ denotes the argument $\x_r$ with $x_i=1, x_j=0, \forall j \in r \setminus \{i\}$, and $\bf{0}$ denotes the argument with $x_j=0, \forall j \in r$.
\end{theorem}
\begin{proof}
Proof is provided in Section \ref{proof_thm_step2}.
\end{proof}

The results derived in Theorem 1 and 2 provide a unified framework for computing the Region approximated fugacities for arbitrary choice of regions. However, one needs to solve the possibly non-convex maximization problem \eqref{eq_opt_step1}, which is a non-trivial problem in general. Hence, in the next section, we first investigate the effect of different choices of regions on the accuracy and complexity of computing RAF. Then, we propose distributed algorithms for some ``useful" choices of regions.

%However, one needs solve the possibly non-convex maximization problem \eqref{eq_opt_step1}. Further, to integrate with CSMA, we should solve \eqref{eq_opt_step1} in a distributed manner. For general choices of regions, it may not possible to meet these requirements. 

%Hence, in the next section, we understand the

%In particular, the feasibility of distributed solution of \eqref{eq_opt_step1} depends on the choice of regions. Hence, we now proceed to understand 


==> Arxiv TMC_journal/model.tex <==
\begin{figure}[h]
\centering
\includegraphics[scale=0.45]{exampl.png} 
%\includegraphics[scale=0.31]{random_graph_new.eps} 
\caption{Example of a small conflict graph consisting of 7 labeled nodes .}
\label{fig_cliq}
\end{figure}
Consider single hop wireless network model as shown in \eqref{fig_cliq}.We consider conflict graph pair wise model where we assume that adjacent nodes cannot transmit together. We want compute fugacities of all the nodes $\{\lt\}_{i=1}^N$ given their service rates $\{s_i\}_{i=1}^N$. We use kikuchi approximation to construct region graph. We use these regions and formulate kikuchi free energy function which can be optimized to obtain approximate set of fugacities for which we achieve service rates.
In kikuchi approach,we begin with an initial set of regions $\{R_0\}$ such that every node $i$ in the network graph is included in atleast one region $r\in{\{R_0\}}$.
 We also make sure that there does not exist a region $r^1$ such that it is subregion of another region $r$ at same level. $$r^1\not\subseteq{r}$$. If there exists such region $r^1$ then it is discarded from $\{R_0\}$. For determination of initial set of regions $\{R_0\}$ with above constraints we have proposed a distributed algorithm which considers maximal cliques as constituents of $\{R_0\}$. We then construct set of regions $\{R_1\}$ by forming all possible intersections of regions in $\{R_0\}$. We make sure no two regions at this level are subregions to one other. This way for construction of set of regions $\{R_2\}$ we take intersections of regions from $\{R_1\}$. We keep doing this to construct regions at different levels till we reach a stage where we cannot go to next level because of no intersections between regions in that level. Finally we obtain a whole set of kikuchi regions $R=\bigcup\limits_{i}R_i$. 
Now we define counting numbers $c_R$ for all the regions in $\{R\}$. For a region $r$ we have counting number $c_r$ as $$c_r=1-\sum_{s\in{S(r)}}c_s$$ where $S(r)$ is set of all regions which are super-regions of region $r$ and belong to $\{R\}$. Counting number ensures that when all the regions are considered together each node effectively accounts only for once.
Let us consider graph in \eqref{fig_cliq} to compute kikuchi regions. For $\{R_0\}$ we consider maximal cliques in the graph which give regions as $\{1,2\}$,$\{2,3,7\}$,$\{2,7,8\}$,$\{3,5,6,7\}$ and $\{3,4\}$. These form $\{R_0\}$. Now we consider their intersections to get $\{R_1\}$. We get intersections like $\{2,7\}$,.. but we also get intersections like $\{2\}$ which are sub-regions of other regions so will be discarded. Finally, we get $\{R_1\}$ regions as $\{2,7\}$ and $\{3,7\}$. Now, we go for $\{R_2\}$ which has only one region $\{7\}$. We cannot go ahead because of no intersections between regions in $\{R_2\}$. Thus we have $R=R_0\cup{R_1\cup{R_2}}$ as illustrated in \eqref{fig_reg} where regions are linked to show dependency. Now, we compute counting numbers $c_R$. For regions in $\{R_0\}$ we have $c_R$ as $1$ because regions in $\{R_0\}$ don not have any super-regions. Then for region $\{2,7\}$ we have $c_R = 1-(1+1) = -1$ since region $\{2,7\}$ has two super-regions from $\{R_0\}$. Similarly,for region $\{3,7\}$ we have $c_R = 1-(1+1) = -1$. For region $\{7\}$ we have $c_R = 1-(1+1+1-1-1) = 0$ as region $\{7\}$ has three super-regions from $\{R_0\}$ and two super-regions from $\{R_1\}$. Now,we have regions $\{R\}$ and their counting numbers $\{c_R\}$.

\begin{figure}[h]
\centering
\includegraphics[scale=0.45]{regions.png} 
%\includegraphics[scale=0.31]{random_graph_new.eps} 
\caption{Region graph level wise for conflict graph in Fig.1}
\label{fig_reg}
\end{figure}

Considering free energy equation for kikuchi regions with counting numbers, we have 
\begin{align}
F=\sum_{r\in{R}}U_r-H_r
\label{eqn_energy_1}
\end{align}
where $U_r$ and $H_r$ are energy and entropy functions for a region $r$ which are given by
\begin{align}
U_r=\sum_{r \in {R}}c_r\sum_{x_r}b_r(x_r)E_r(x_r)
\label{eqn_energy_2}
\end{align}
and
\begin{align}
H_r=-\sum_{r \in {R}}c_r{x_r}b_r(x_r)log b_r(x_r)
\label{eqn_energy_3}
\end{align}
Using \eqref{eqn_energy_2} and \eqref{eqn_energy_3} in \eqref{eqn_energy_1},we have kikuchi free energy as
\begin{align}
F_K= \sum_{r \in {R}}c_r\left( \sum_{x_r}b_r(x_r)E_r(x_r) + \sum_{x_r}b_r(x_r)log b_r(x_r)\right)
\label{eqn_energy_4}
\end{align}

==> Arxiv TMC_journal/neighbourhood.tex <==
In this section, we propose a region-based approximation that improves the error beyond the clique-based approach, without explicitly using the information about the two-hop neighbours. The key idea is to use the fact that our results derived in Theorem \ref{thm_step1}, \ref{thm_step2} hold for any collection of regions, and go beyond the standard Kikuchi approximation / Cluster variation method based regions. Specifically, our collection of regions $\Re$ includes
\begin{itemize}
\item For each vertex, $i \in V$, we include a neighbourhood region $r=\N_i$.
\item All the clique based regions.
\end{itemize}
The counting numbers are computed using \eqref{eq_counting_formula}.

\noindent \emph{Remark:} This collection of $\Re$ does not fall under the Kikuchi approximation framework since our $\Re$ may not include the intersections of the neighbourhood regions.

Let $\Re_N$ denote the set of all the neighbourhood regions, and $\Re_C$ denote the set of all the clique regions in $\Re$. In the following theorem we show that the optimization problem \eqref{eq_opt_step1} decouples into local optimization problems at each neighbourhood.
\begin{theorem}
Let the collection of regions $\Re$ include the neighbourhood regions $\Re_{N}$, and all the clique regions $\Re_{C}$. Let $\{s_i\}$ be the required service rates. Let $\{b_r\}$ be the solution of the optimization problem \eqref{eq_opt_step1}. For any $r \in \Re_{C}$, the corresponding regional distribution $b_r^*$  is given by \eqref{eq_reg_dist}. For any $r \in \Re_N$, the corresponding $b_r^*$ is given by the following optimization problem:
\begin{align}
 \underset{b_r}{\arg \max} & \; H_r(b_r), \; \; \text{subject to} \label{eq_opt_neigh}\\
\sum_{x_r \in \I_r : x_i=1} b_r (x_r) &= s_i, \; \; \; i \in r.
 \end{align}
\end{theorem}
\begin{proof}
As discussed in Theorem \ref{thm_clique}, the regional $b_r^*$ of a clique are explicitly determined by the service rates. Further, 
\end{proof}

==> Arxiv TMC_journal/numerical_results.tex <==


\begin{figure*}
\begin{minipage}{.33 \textwidth}
\centering
\includegraphics[scale=0.34]{complete_graph.pdf} 
%\includegraphics[scale=0.53]{sq_good_graph.eps} 
\caption{Complete graph}
\label{fig_complete}
\end{minipage}
\begin{minipage}{.33 \textwidth}
\centering
\includegraphics[scale=0.45]{grid_graph.pdf} 
%\includegraphics[scale=0.53]{sq_good_graph.eps} 
\caption{Grid graph}
\label{fig_grid}
\end{minipage}
\begin{minipage}{.33 \textwidth}
\centering
\includegraphics[scale=0.55]{Exact3_graph.pdf} 
\caption{Chordal graph}
\label{fig_chordal}
\end{minipage}
\end{figure*}

\begin{figure*}
\begin{minipage}{.33 \textwidth}
\centering
\includegraphics[scale=0.42]{complete_prac.pdf} 
%\includegraphics[scale=0.53]{sq_good_graph.pdf} 
\caption{Error plot for Complete graph}
\label{fig_complete_prac}
\end{minipage}
\begin{minipage}{.33 \textwidth}
\centering
\includegraphics[scale=0.44]{grid_prac.pdf} 
%\includegraphics[scale=0.53]{sq_good_graph.pdf} 
\caption{Error plot for grid graph}
\label{fig_grid_prac}
\end{minipage}
\begin{minipage}{.33 \textwidth}
\centering
\includegraphics[scale=0.42]{Exact3_practical.pdf} 
\caption{Error plot for chordal graph}
\label{fig_chordal_prac}
\end{minipage}
\caption*{The approximation error is plotted as function of the network load for the three topologies considered above}
\end{figure*}



%\begin{figure*}
%\begin{minipage}{.33 \textwidth}
%\centering
%%\includegraphics[scale=0.535]{sq_two_pent_graph.pdf} 
%\includegraphics[scale=0.46]{20_graph_3.pdf}
%\caption{Random graph}
%\label{fig_random}
%\end{minipage}
%\begin{minipage}{.33 \textwidth}
%\centering
%%\includegraphics[scale=0.535]{sq_two_pent_graph.pdf} 
%\includegraphics[scale=0.42]{20_mat_3_prac.pdf}
%\caption{Error plot for random graph}
%\label{fig_random_prac}
%\end{minipage}
%\end{figure*}

\begin{figure*}
\begin{minipage}{.33 \textwidth}
\centering
\includegraphics[scale=0.39]{15_graph_n1.pdf} 
%\includegraphics[scale=0.53]{sq_good_graph.pdf} 
\caption{15-link random topology}
\label{fig_random15}
\end{minipage}
\begin{minipage}{.33 \textwidth}
\centering
\includegraphics[scale=0.465]{20_graph_n2.pdf} 
%\includegraphics[scale=0.53]{sq_good_graph.pdf} 
\caption{20-link random topology}
\label{fig_random20}
\end{minipage}
\begin{minipage}{.33 \textwidth}
\centering
\includegraphics[scale=0.43]{25_graph_n1.pdf} 
\caption{25-link random topology}
\label{fig_random25}
\end{minipage}
\end{figure*}

\begin{figure*}
\begin{minipage}{.33 \textwidth}
\centering
\includegraphics[scale=0.45]{15_abs_n1.pdf} 
%\includegraphics[scale=0.53]{sq_good_graph.pdf} 
\caption{Error for 15-link topology}
\label{fig_r15_abs}
\end{minipage}
\begin{minipage}{.33 \textwidth}
\centering
\includegraphics[scale=0.45]{20_abs_n2.pdf} 
%\includegraphics[scale=0.53]{sq_good_graph.pdf} 
\caption{Error for 20-link topology}
\label{fig_r20_abs}
\end{minipage}
\begin{minipage}{.33 \textwidth}
\centering
\includegraphics[scale=0.45]{25_abs_n1.pdf} 
\caption{Error for 25-link topology}
\label{fig_r25_abs}
\end{minipage}
\caption*{The approximation error is plotted as function of the network load for 3 random topologies }
\end{figure*}






\emph{Simulation Setting:}
We first provide simulation results for complete graph, grid graph, and chordal graph (Figure \ref{fig_complete}- \ref{fig_chordal}) topologies. Further, we consider some random topologies of different sizes (Figure \ref{fig_random15} - \ref{fig_random25}). Specifically, we generate random geometric graphs on a two-dimensional square of length three. Two vertices are connected by an edge if they are within a distance of $0.8$. We consider symmetric service rate requirements for all the links\footnote{There is no specific reason to choose these parameters. The performance of the algorithms is qualitatively similar for other choices of parameters too.}.
 
 \subsection*{Approximation error}
We define the approximation error $e(s^t)$, as the maximum deviation from the required service rate. In particular, for a given target service rate vector $s^t=[s_i^t]_{i=1}^N$, $e(s^t)=\max\limits_{i}  \;|s^t_i - s^a_i| , $ where, $s^a=[s_i^a]_{i=1}^N$ are the service rates supported by using the approximated fugacities $\{\vt\}_{i=1}^N$. We vary the load (the ratio of the required service rate to the maximum permissible service rate) of the network by increasing the required service rates, and plot the percentage error. We compared the accuracy of our algorithms with the existing Bethe approximation based algorithm \cite{bethe_jshin}. 

\emph{Chordal graph:}
As proved in Theorem \ref{thm_chordal}, our algorithm is exact if the underlying conflict graph is chordal. This result is verified using a complete graph topology (which is trivially a chordal graph) and another chordal graph shown in Figure \ref{fig_chordal}. As shown in Figures \ref{fig_complete_prac}, \ref{fig_chordal_prac}, the Bethe approximation based algorithm incurs an error of about $20$ percent when the network is operated at the maximum capacity, while our Clique based algorithm is exact. 

\emph{Grid graph:} For the grid graph, the error is plotted in Figure \ref{fig_grid_prac}. Since, there are no cliques other than the trivial edges and vertices, the Bethe approximation and the Clique based algorithm will coincide. Both these algorithms incur an error of about $22$ percent at a load of $0.7$. However, our  4-cycle based algorithm is accurate with an error of about $1$ to $2$ percent.




\emph{Random graphs:} We considered three random graphs of sizes 15, 20 and 25 as shown in Figure \ref{fig_random15} - \ref{fig_random25}. We plotted the corresponding approximation errors in Figure \ref{fig_r15_abs} - \ref{fig_r25_abs}. It can be observed that the proposed algorithms perform significantly better than the Bethe approximation. In particular, for the twenty link topology at a load of $0.8$, the Bethe approximation has an error of about 28 percent, while our clique based and 4-cycle based algorithms have an error of about 9 and 7 percent respectively. Further, for the 15, 25 link topologies, when the Bethe approximation has an error of about 20 percent, the clique based approach incurs less than 2 percent error. Moreover, the 4-cycle based approach is almost exact with error close to zero. 

%\begin{table}
%\begin{center}
%\resizebox{\columnwidth}{!}{%
%  \begin{tabular}{|c | c | c| c |}
%  \hline
%  Algorithm & Minimum  & Maximum  & Average  \\  
%     &error $\%$& error $\%$ & error $\%$ \\ 
%    \hline
%Bethe  & 19.1 & 30.46 & 25.63 \\   
%Clique-based & 0 & 8.94 & 2.78  \\
%4-cycle based & 0& 6.24 & 1.83  \\
%    \hline
%     \end{tabular}}
% \caption{The results obtained by simulating random topologies of size 20 at a load of $0.8$.}
%  \label{table_error}
%  \end{center}
% 
%   \end{table}
To present the average behaviour of the error, we considered thirty randomly generated topologies of size $20$, and observed the error when the required service rates are set to a load of $0.8$. We have presented the average error obtained across these topologies. As observed from Table \ref{table_error}, our algorithms have a significantly better error performance.

\begin{table}
\begin{center}

  \begin{tabular}{|c | c | }
  \hline
  Algorithm &  Average  \\  
     & error $\%$ \\ 
    \hline
Bethe  &  25.63 \\   
Clique-based & 2.78  \\
4-cycle based &1.83  \\
    \hline
     \end{tabular}
 \caption{The results obtained by simulating random topologies of size 20 at a load of $0.8$.}
  \label{table_error}
  \end{center}
 
   \end{table}






%This is the typical behaviour for most of the topologies that we have considered.

\noindent \emph{Remark on complexity}: The Bethe approximation \cite{bethe_jshin} uses only the service rates of the neighbours to compute the fugacities, and hence the error is significantly large. Our algorithms result in better error performance at the additional cost of obtaining the local topology information. Specifically, our clique-based algorithm requires the topology of the one-hop neighbourhood to compute the clique regions. The 4-cycle based algorithm requires the information of two-hop neighbourhood topology to compute the 4-cycle regions. Since the complexity of our algorithms just depend on the size of the local neighbourhood, the complexity does not scale with the network size, when the average density of the network is constant. On the other hand, stochastic gradient descent based algorithms \cite{libin} that converge to the exact fugacities, incur an exponentially slow convergence rate in the size of the network. 

\section{Conclusions}
The problem of computing the optimal fugacities for Gibbs sampling based CSMA algorithms is NP-hard. In this work, we derived estimates of the fugacities by using a framework called the \emph{regional free energy approximations}. Specifically, we derived explicit expressions for approximate fugacities corresponding to a given feasible service rate vector. We further proved that our approximate fugacities are exact for the class of \emph{chordal} graphs.  A distinguishing feature of our work is that the regional approximations that we proposed are tailored to conflict graphs with small cycles, which is a typical characteristic of wireless networks. Numerical results indicate that the fugacities obtained by the proposed methods are quite accurate, and significantly outperform the existing Bethe approximation based techniques.


%\subsection{Delay performance}
%\begin{figure}
%\includegraphics[scale=0.45]{comparision_que.pdf}
%\caption{Comparison of Queue lengths for the Bethe approximation and the 4-cycle based approach for a $4 \times 4$ grid topology}
%\label{fig_queues}
%\end{figure}
%Now, we compare the delay performance of the Bethe approximation and our regional approximation using a $4 \times 4$ grid (torus) topology. We operate the network at a load of $55$ percent (which corresponds to a symmetric arrival rate of $0.27$ at each link).  We use the formulas derived in Theorem \ref{thm_grid_formula}, Corollary \ref{cor_bethe} to compute the fugacities for the 4-cycle based approach, and the Bethe approximation respectively. We assume that each link has a Bernoulli arrival process, and run the CSMA algorithm to schedule the links. The evolution of the queue length per link is plotted in Figure \ref{fig_queues}. The Bethe approximation results in a steady state queue length of about $10^5$ while the 4-cycle based approach has a lower queue length of $10^3$, which is desirable.
%
%The reason for this improvement can be understood by comparing the fugacities of these two approaches. Specifically, the Bethe approximation corresponds to a fugacity of $14.8$, while the 4-cycle based approach corresponds to a fugacity of $1.6$. It is known that higher fugacities lead to poor delay performance due to a phenomenon called the \emph{temporal starvation} \cite{marbach}. Here, the Bethe approximation overestimates the fugacity value, thereby resulting in higher delay / queue length. 











==> Arxiv TMC_journal/preliminaries.tex <==
\subsection{Product form distribution}
Let $S$ be a finite set, and let $X_i, i=1, 2, \dots, N$, be random variables each taking values in $S$. The joint PMF (probability mass function) of the random variables is succinctly denoted as $p(\x)$, where $\x=\{x_1,x_2, \dots, x_N \}$. Suppose that $p(\x)$ factors into a product of $M$ functions and is given by,
\begin{align}
p(\x)&= \frac{1}{Z} \prod\limits_{j=1}^M f_j(\x_j), \hspace{0.7cm} \x \in S^N.  \label{eq_factors}
\end{align}
The function $f_j(\cdot)$ has arguments $\x_j$ that are some non-empty subset of $\{x_1,x_2, \dots, x_N \}$. Here $Z$ is a normalization constant. Further, the product form distributions are generally represented using a graph called factor graph \cite{book_martin} that has two sets of nodes namely variable nodes and factor nodes corresponding to the variables and the functions in \eqref{eq_factors} respectively. An edge is drawn between a variable node and a factor node if the variable is an argument of that factor function.
\begin{comment}
\textbf{Factor graph:}
A factor graph \cite{yedidia} is a bipartite graph used to visualize the factorization structure of the joint distribution \eqref{eq_factors}. The factor graph has two sets of nodes called the \emph{variable nodes} and the \emph{factor nodes} corresponding to the variables and the functions in \eqref{eq_factors} respectively. The variable nodes are represented using circles while the factor nodes are represented using squares. An edge is drawn between a variable node and a factor node if the variable is an argument of that factor function.
  Let us now consider an example.\\
\begin{figure}
{
\begin{center}
\begin{tikzpicture}[scale=0.3]
%\draw (0,0) -- (-2,0.7);
%\draw (-2,-0.7) -- (0,0);
\draw (0,0) -- (0.7,0);
\draw (0.7,0) -- (0.7,0.7);
\draw (0.7,0.7) -- (0,0.7);
\draw (0,0.7) -- (0,0);
\node at (0.35,-0.7) {{$f_1$}};

\draw (2,0) -- (2.7,0);
\draw (2.7,0) -- (2.7,0.7);
\draw (2.7,0.7) -- (2,0.7);
\draw (2,0.7) -- (2,0);
\node at (2.35,-0.7) {{$f_2$}};

\draw (4,0) -- (4.7,0);
\draw (4.7,0) -- (4.7,0.7);
\draw (4.7,0.7) -- (4,0.7);
\draw (4,0.7) -- (4,0);
\node at (4.35,-0.7) {{$f_3$}};


\draw (-1.5,3)circle(0.4cm);
\node at (-1.5,4) {{$x_1$}};
\draw (0.5,3)circle(0.4cm);
\node at (0.5,4) {{$x_2$}};
\draw (2.5,3)circle(0.4cm);
\node at (2.5,4) {{$x_3$}};
\draw (4.5,3)circle(0.4cm);
\node at (4.5,4) {{$x_4$}};
\draw (6.5,3)circle(0.4cm);
\node at (6.5,4) {{$x_5$}};
%\node at (3,0.85+0.2) {$2$};





\draw (0.35,0.7) -- (-1.5,3-0.4); %A- x1
\draw (0.35,0.7) -- (0.5,3-0.4); %A- x2
\draw (0.35,0.7) -- (6.5,3-0.4); %A- x5

\draw (2.35,0.7) -- (0.5,3-0.4); %B- x2
\draw (2.35,0.7) -- (4.5,3-0.4); %B- x4

%\draw (4.35,0.7) -- (-1.5,3-0.4); %C- x1
\draw (4.35,0.7) -- (2.5,3-0.4); %C- x3
\draw (4.35,0.7) -- (6.5,3-0.4); %C- x5
\end{tikzpicture}
\end{center}
}
\vspace{-0.6cm}
\caption{Factor graph}
\label{fig_fg}
\end{figure}
\emph{Example} (A simple factor graph): Consider a simple distribution of the form
\begin{align*}
p(x_1,x_2,x_3,x_4,x_5)&= \frac{1}{Z} f_1(x_1, x_2 , x_5) f_2(x_2, x_4) f_3(x_3, x_5).
\end{align*}
Using the notation in \eqref{eq_factors}, the distribution can be succinctly represented as
\begin{align*}
p(\x)&= \frac{1}{Z} f_1(\x_1) f_2(\x_2) f_3(\x_3), 
\end{align*}
where, $\x=\{x_1, x_2, x_3, x_4, x_5 \}$, $\x_1=\{x_1, x_2,  x_5 \}$, $\x_2=\{ x_2,  x_4 \}$, $\x_3=\{x_3,  x_5 \}$. The factor graph corresponding to this example is shown in Figure \ref{fig_fg}.\\
\end{comment}
For the product form distribution considered in \eqref{eq_factors}, we are interested in the marginal probabilities called variable marginals and factor marginals.

\noindent \emph{Variable node marginals: }
The marginal probability distribution $p_i({x_i})$ corresponding to a variable node $i$, is obtained by summing $p(\x)$ over the variables corresponding to all other variable nodes, \ie, $p_i({x_i})= \sum_{\x \setminus x_i} p(\x)$, $x_i \in S$, $ i=1,\dots, N.$

\noindent \emph{Factor node marginals:} Corresponding to each factor node, $j=1, \dots, M$, the marginal probability function $\p_j({{\x}_j})$,  is obtained by summing $p(\x)$ over all the variables in $\x \setminus {\x}_j$. Let $N_j$ denote the number of arguments in $f_j$, \ie, $N_j= |\x_j|$. Then, 
$
\p_{j}({{\x}_j}) = \sum_{\x \setminus {\x}_j} p(\x)$, ${\x}_j \in S^{N_j}.$

Let $\pv:=\{p_i\}_{i=1}^N$, $\pn:=\{\p_j\}_{j=1}^M$ denote the collection of all the variable node marginals and  the factor node marginals corresponding to the distribution $p(\x)$ respectively. Next, we discuss the Bethe approximation \cite{book_martin} which is used to estimate these marginal probability distributions.
\subsection{Bethe approximation}
%One approach to computing the partition function corresponding to the distribution $p(\x)$,  is to minimize a function called Gibbs free energy (GFE) over all the valid probability distributions on the state space $S^N$. However, as $N$ becomes large, even this procedure is intractable, as the optimization variables take exponentially large memory to store. We hence take recourse to the Bethe approximation, which is an approximate, but a more practical technique to estimate the marginals explicitly \cite{yedidia} . Next, we introduce the concepts of Bethe free energy and Bethe optimization with focus on the application for CSMA networks. 
\subsubsection{Bethe free energy (BFE)}
Consider a probability distribution $p(\x)$ of the form \eqref{eq_factors} for which we are interested in finding the marginals. Let $b(\x)$ be some distribution on $S^N$, whose factor and variable marginals are given by $\bn=\{\b_j\}_{j=1}^M$ and $\bv=\{b_i\}_{i=1}^N$. Here, $p(\x)$ is referred to as the \emph{true} distribution, and $b(\x)$ is referred to as the \emph{trial} distribution as it is used to estimate the true distribution $p(\x)$. Next, we define the Bethe entropy, which is required for the definition of BFE. The Bethe entropy of a distribution $b(\x)$ is a weighted sum of the entropies corresponding to the factor and the variable marginal distributions of $b(\x)$ and is given by $H_B\left( \bn, \bv \right)
=\sum_{j=1}^M \H_j(\b_j) - \sum_{i=1}^N (d_i-1) H_i(b_i)$,
%\begin{align*}
%H_B\left( \bn, \bv \right)
%&=\sum\limits_{j=1}^M \H_j(\b_j) - \sum\limits_{i=1}^N (d_i-1) H_i(b_i), 
%\end{align*}
where $d_i$ is the degree of the variable node $i$ in the factor graph, and $\H_j(\b_j)= -\sum_{y \in S^{N_j}} \b_j(y) \ln \b_j(y)$, $
H_i(b_i)= -\sum_{y \in S} b_i(y) \ln b_i(y)$ denote the entropies of the factor marginal $\b_j(\x_j)$, and the variable marginal $b_i(x_i)$ respectively.
\begin{definition}
Consider a true distribution $p(\x)$ of the form \eqref{eq_factors}. Let $b(\x)$ be a trial distribution. Then, the Bethe free energy $F_B(b)$ is defined as
\begin{align}
F_B(b)&=F_B\left( \bn, \bv \right)=U_B(\bn, \bv) - H_B(\bn, \bv),  \label{eq_bfe_eg}
\end{align}
where $U_B(\bn, \bv)=-\sum_{j=1}^M \sum_{\x_j}  \b(\x_j) \ln f_j(\x_j)$.
\end{definition}

 \subsubsection{Bethe optimization (BO)}
The following optimization problem is referred to as the Bethe optimization.
\begin{align}
&\underset{\bn, \bv} {\arg \min}\; \;  F_B(\bn, \bv), \text{  subject to}  \label{eq_bethe_min}\\
 b_i(x_i) &\geq 0, \hspace{0.4cm} i = 1, \dots, N, \; \;  x_i \in S,\nonumber\\ 
  \sum_{x_i} b_{i} (x_i)&=1, \hspace{0.4cm} i = 1, \dots, N, \nonumber\\ 
\b_j(\x_j) &\geq 0, \hspace{0.4cm} j = 1, \dots, M, \; \;   \x_j \in S^{N_j},\nonumber\\
 \sum_{\x_j} \b_{j} (\x_j)&=1, \hspace{0.4cm} j = 1, \dots, M, \nonumber\\
 \sum_{\x_j \setminus \{x_i \}} \b_j(\x_j)&= b_i(x_i), \hspace{0.2cm} j=1, \dots, M, \; i \in \N_j,\; x_i \in S ,\nonumber
\end{align}
where $\N_j$ is the set of indices of all the variable nodes associated with the factor node $j$.

\emph{Note:}
A feasible collection $(\bn,\bv)$ of the Bethe optimization problem does not necessarily represent the marginals of any coherent joint distribution over $S^N$, and are therefore referred to as \emph{pseudo-marginals} \cite{book_martin}. In spite of performing the optimization over a relaxed set, the solution of the Bethe optimization $(\bn^*, \bv^*)$ exactly coincides with the marginals of the true distribution $(\pn^*, \pv^*)$, if the underlying factor graph is a tree. Further, for factor graphs with loops, the solution leads to very good estimates of the true marginals \cite{book_martin,bethe_emprical}. In fact, in many applications, solving for the global minimizer of \eqref{eq_bethe_min} is not feasible because of its non-convexity. Hence, a stationary point of the BFE satisfying the constraints in \eqref{eq_bethe_min} is considered as a good estimate of the true marginals \cite{book_martin}.


\subsection{Bethe approximation for CSMA}
We observe that the stationary distribution of the CSMA Markov chain $p(\x)$ given by \eqref{eq_succint} is in product from \eqref{eq_factors} with the factor functions $\{f_j \}_{ j=1}^N$ defined as
\begin{align}
f_j(\x_j)= \begin{cases}
\lambda_j, & \text{if }  x_j=1, \gamma_j(\x_j) \geq T, \label{eq_local_factors} \\
  0, & \text{if } x_j=1, \gamma_j(\x_j) < T, \\
 1,  & \text{if } x_j = 0.
\end{cases}
\end{align}
where $\x_j$ is the local schedule of the link $j$ defined earlier.

\begin{comment}
 Using these factor functions, $p(\x)$ can be equivalently represented as
\begin{align}
p(\x)&= \frac{1}{Z}\prod\limits_{j=1}^N f_j(\x_j),  \hspace{0.7cm} \x \in \{0,1\}^\N. \label{eq_dist_prod1}
\end{align}

Next, let us consider the factor graph representation of $p(\x)$. Observe that in $p(\x)$, the number of factor functions are equal to the number of variables nodes $N$, \ie, corresponding to each variable node $j$, there is a factor node $f_j$. For example, if we consider a network with the interference graph (defined in Section \ref{sec_model}) given by Figure \ref{fig_randomgraph}, then the corresponding factor graph is given by Figure \ref{fig_fg_sinr}. 
\end{comment}

By the definition of local feasibility, $p(\x)$ assigns zero probability to a schedule $\x$, if it is locally infeasible at any link. Hence, the factor node marginals $\pn = \{\p_j\}_{j=1}^N$ have to satisfy $\p_j(y)=0, \; \; \; \forall y \notin \I_j, \;  \forall j \in \N.$

\begin{comment}
If we recall the definition of local feasibility, it can be observed that the distribution $p(\x)$ assigns zero probability to a schedule $\x$, if it is locally infeasible at any link $j \in \N$. Hence, the factor node marginals $\pn = \{\p_j\}_{i=1}^N$ have to satisfy  
\begin{align}
\p_j(y)&=0, \; \; \; \forall y \notin \I_j, \;  \forall j \in \N. \label{eq_local_feasibility}
\end{align}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
       \begin{tikzpicture}[scale=0.2]
%\draw (0,0) -- (-2,0.7);
%\draw (-2,-0.7) -- (0,0);
%\draw (1.65,3.65) -- (2.35,3.65);
%\draw (1.65,4.35) -- (2.35,4.35);
%\draw (1.65,3.65) -- (1.65,4.35);
%\draw (2.35,3.65) -- (2.35,4.35);
%\node at (1.0,4) {{$f_{23}$}};
%
%\draw (4-.35,4.5-.35) -- (4+.35,4.5-.35);
%\draw (4-.35,4.5+.35) -- (4+.35,4.5+.35);
%\draw (4-.35,4.5-.35) -- (4-.35,4.5+.35);
%\draw (4+.35,4.5-.35) -- (4+.35,4.5+.35);
%\node at (4,5.5) {{$f_{35}$}};
%
%
%\draw (4-.35,2.5-.35) -- (4+.35,2.5-.35);
%\draw (4-.35,2.5+.35) -- (4+.35,2.5+.35);
%\draw (4-.35,2.5-.35) -- (4-.35,2.5+.35);
%\draw (4+.35,2.5-.35) -- (4+.35,2.5+.35);
%\node at (4,1.5) {{$f_{25}$}};
%
%
%\draw (8-.35,5.5-.35) -- (8+.35,5.5-.35);
%\draw (8-.35,5.5+.35) -- (8+.35,5.5+.35);
%\draw (8-.35,5.5-.35) -- (8-.35,5.5+.35);
%\draw (8+.35,5.5-.35) -- (8+.35,5.5+.35);
%\node at (8,6.5) {{$f_{15}$}};
%
%
%\draw (8-.35,1.5-.35) -- (8+.35,1.5-.35);
%\draw (8-.35,1.5+.35) -- (8+.35,1.5+.35);
%\draw (8-.35,1.5-.35) -- (8-.35,1.5+.35);
%\draw (8+.35,1.5-.35) -- (8+.35,1.5+.35);
%\node at (8,0.5) {{$f_{45}$}};


\draw (2,2)circle(0.4cm);
\node at (1.2,0.9) {{$2$}};
\draw (2,6)circle(0.4cm);
\node at (1.3,7) {{$3$}};
\draw (6,3)circle(0.4cm);
\node at (6.1,4.4) {{$5$}};
\draw (10,8)circle(0.4cm);
\node at (10.7,9) {{$1$}};
\draw (10,-0)circle(0.4cm);
\node at (10.8,-0.7) {{$4$}};
%\node at (3,0.85+0.2) {$2$};



\draw (6+0.2,3-0.2) -- (10-0.2,0+0.35); %3-5
%\draw (10-0.2,0+0.35) -- (8+.35,1.5-.35); %3-5

\draw (10-0.2,8-0.2) -- (6+0.2,3+0.2); %4-3
%\draw (6+0.2,3+0.2) -- (8-.35,5.5-.35); %3-4

\draw (6-0.2,3-0.2) -- (2+0.2,2+0.2); %3-1
%\draw (2+0.2,2+0.2) -- (4-.35,2.5-0); %1-3

\draw (6-0.2,3+0.2) -- (2+0.2,6-0.2); %3-1
%\draw (2+0.2,6-0.2) -- (4-.35,4.5+.35); %1-3

\draw (2,2+0.4) -- (2,6-0.4); %3-1
%\draw (2,6-0.4) -- (2,4+.35); %1-3
\end{tikzpicture}
\caption{interference graph}
\label{fig_randomgraph}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
       \begin{tikzpicture}[scale=0.3]
\draw (-1.5,3)circle(0.4cm);
\node at (-1.5,4) {{$x_2$}};

\draw (0.5,3)circle(0.4cm);
\node at (0.5,4) {{$x_3$}};

\draw (2.5,3)circle(0.4cm);
\node at (2.5,4) {{$x_5$}};
\draw (4.5,3)circle(0.4cm);
\node at (4.5,4) {{$x_1$}};
\draw (6.5,3)circle(0.4cm);
\node at (6.5,4) {{$x_4$}};
%\node at (3,0.85+0.2) {$2$};

\draw (-1.5-.35,0-.35) -- (-1.5+.35,0-.35);
\draw (-1.5-.35,0+.35) -- (-1.5+.35,0+.35);
\draw (-1.5-.35,0-.35) -- (-1.5-.35,0+.35);
\draw (-1.5+.35,0-.35) -- (-1.5+.35,0+.35);
\node at (-1.5,-1) {{$f_{2}$}};

\draw (0.5-.35,0-.35) -- (.5+.35,0-.35);
\draw (0.5-.35,0+.35) -- (.5+.35,0+.35);
\draw (0.5-.35,0-.35) -- (.5-.35,0+.35);
\draw (0.5+.35,0-.35) -- (.5+.35,0+.35);
\node at (.5,-1) {{$f_{3}$}};

\draw (2.5-.35,0-.35) -- (2.5+.35,0-.35);
\draw (2.5-.35,0+.35) -- (2.5+.35,0+.35);
\draw (2.5-.35,0-.35) -- (2.5-.35,0+.35);
\draw (2.5+.35,0-.35) -- (2.5+.35,0+.35);
\node at (2.5,-1) {{$f_{5}$}};

\draw (4.5-.35,0-.35) -- (4.5+.35,0-.35);
\draw (4.5-.35,0+.35) -- (4.5+.35,0+.35);
\draw (4.5-.35,0-.35) -- (4.5-.35,0+.35);
\draw (4.5+.35,0-.35) -- (4.5+.35,0+.35);
\node at (4.5,-1) {{$f_{1}$}};

\draw (6.5-.35,0-.35) -- (6.5+.35,0-.35);
\draw (6.5-.35,0+.35) -- (6.5+.35,0+.35);
\draw (6.5-.35,0-.35) -- (6.5-.35,0+.35);
\draw (6.5+.35,0-.35) -- (6.5+.35,0+.35);
\node at (6.5,-1) {{$f_{4}$}};



\draw (-1.5,0.35) -- (-1.5,3-0.4); %A- x1
\draw (0.5,0.35) -- (0.5,3-0.4); %B- x2
\draw (2.5,0.35) -- (2.5,3-0.4); %B- x2
\draw (4.5,0.35) -- (4.5,3-0.4); %B- x2
\draw (6.5,0.35) -- (6.5,3-0.4); %B- x2

%for node 2
\draw (-1.5,0.35) -- (0.5,3-0.4); %A- x1
\draw (-1.5,0.35) -- (2.5,3-0.4); %A- x1

%for node 2
\draw (0.5,0.35) -- (-1.5,3-0.4); %A- x1
\draw (0.5,0.35) -- (2.5,3-0.4); %A- x1

%for node 5
\draw (2.5,0.35) -- (0.5,3-0.4); %A- x1
\draw (2.5,0.35) -- (-1.5,3-0.4); %A- x1
\draw (2.5,0.35) -- (4.5,3-0.4); %A- x1
\draw (2.5,0.35) -- (6.5,3-0.4); %A- x1

%for node 1
\draw (4.5,0.35) -- (2.5,3-0.4); %A- x1

%for node 4
\draw (6.5,0.35) -- (2.5,3-0.4); %A- x1

\end{tikzpicture}
\caption{Factor graph}
\label{fig_fg_sinr}
    \end{subfigure}
    \caption{Graphs associated with the SINR model}
\end{figure}
\end{comment}
\textbf{BFE for CSMA:}
We shall consider the product form representation of the CSMA stationary distribution $p(\x)$ in \eqref{eq_succint} and compute the BFE. As defined in \eqref{eq_bfe_eg}, the BFE for a given trial distribution $b(\x)$ has two terms $U_B(\bn,\bv)$, $H_B(\bn, \bv)$. The following lemma characterizes the first term $U_B(\bn, \bv)$.
\begin{lemma} \label{lemma_u_bethe}
If the factor marginals of a trial distribution $\bn$, assign zero probabilities to all the infeasible local schedules, \ie, 
 \begin{align}
 \b_j(y)=0, \;  \forall y \notin \I_j, \;  \forall j \in \N, \label{eq_bn_feasible}
 \end{align}
then $U_B(\bn, \bv)$ reduces to $U_B(\bn, \bv)=$ $U_B(\bv)= -\sum_{i=1}^N b_i(1) \ln\lambda_i.$ Moreover, if $\bn$ does not satisfy \eqref{eq_bn_feasible}, $U_B(\bn, \bv)=  \infty$.
\end{lemma}
\begin{proof}
Proof follows from definition of factors in \eqref{eq_local_factors}.
\end{proof}
%\begin{align*}
%U(b)&= -\sum\limits_{\ds \in \{0,1\}^\N} b(\ds) E(\ds), \\
%&=-\sum\limits_{\ds \in \{0,1\}^\N} b(\ds) .\left(-\sum\limits_{a=1}^N \mu_a \left( \ds(\bar{\N_a}) \right)\log(\lambda_a)\right),  \\
%&=-\sum\limits_{a=1}^N \left(\sum\limits_{\dnaa \in \{0,1\}^{\naa}} \mu_a\left( \dnaa \right)b_{\naa}\left(\dnaa\right) \right)\log(\lambda_a),\\
%&= -\sum\limits_{a=1}^N \log(\lambda_a) \E_{b_{\naa}}[\mu_a], \\
%&= -\sum\limits_{a=1}^N \log(\lambda_a) b_a(1).
%\end{align*}

Using Lemma \ref{lemma_u_bethe} and \eqref{eq_bfe_eg}, the BFE for any $(\bn, \bv)$ that satisfies \eqref{eq_bn_feasible} is given by
\begin{align}
F_B(\bn,\bv)&=F_B\left( \{\b_j\}_{j=1}^N,  \{b_i\}_{i=1}^N \right),  \label{eq_bfe}\\
&= \sum\limits_{i=1}^N  -b_i(1) \ln\lambda_i  - \H_i(\b_i)  +  (d_i-1) H_i(b_i), \nonumber
\end{align}
where $d_i$ is degree of variable node $i$ in the factor graph. For $(\bn, \bv)$ that does not satisfy \eqref{eq_bn_feasible}, $F_B(\bn, \bv) = \infty$.


==> Arxiv TMC_journal/preliminaries_rfe.tex <==
We introduce the notion of Regional free energy (RFE), which is useful in finding accurate estimates of the marginals of a distribution like $p(\x)$ in \eqref{eq_dist}. We require the following definitions to introduce RFE \cite{book_martin}, \cite{v_anant_kik}, \cite{yedidia}. 


%\emph{Product form distribution:}
%Let $X_i, i=1, 2, \dots, N$ be random variables each taking values in a finite set $S$. Let $p(\x)$ denote the joint distribution (Probability mass function) of these variables random variables, where $\x=\{x_1,x_2, \dots, x_N \}$. Suppose that the distribution $p(\x)$ factors into a product of $M$ functions, and is given by
%\begin{align}
%p(\x)&= \frac{1}{Z} \prod\limits_{a=A}^M f_a(\x_a), \hspace{0.7cm} \x \in S^N.  \label{eq_factors}
%\end{align}
%Here the index $a$ varies over $\{A,B \dots, M\}$ to correspond to the functions $f_A, f_B, \dots, f_M$. The function $f_a(\cdot)$ has arguments $\x_a$ that are some non-empty subset of $\x=\{x_1,x_2, \dots, x_N \}$. Here $Z$ is a normalization constant. 
%
%\emph{Region:} A region $r$ is any set of variables and factors, such that if a factor belongs to the region, all the variables involved in that factor are also present in the region. 
%
%Now, we consider two examples and explain the definition of region. 
%
%\noindent \emph{Example 1:}
%Consider the product form distribution
%\begin{align*}
%p(x_1,x_2,x_3,x_4,x_5)= f_A(x_1, x_2 , x_5) f_B(x_2, x_4) f_C(x_3, x_4).
%\end{align*}
%Then $r=\{B, C, 2, 3, 4,5\}$ is a valid region with factors $B,C$, and variables $2,3,4,5$. To verify that this is a valid region, for each factor we should check if its variables are present in that region. Specifically observe that for factor $B$,  its variables $2,4$ are included, and for factor $C$ its variables $3,4$ are also included. Note that presence of variable $5$ is allowed since, there is no restriction on having additional variables. For example, even a region $r=\{4\}$ is also a valid region. However, a region $r=\{B,2\}$ is not valid because, when $B$ is included in a region, all its variables $2,4$ should be included.
%
%\noindent \emph{Example 2:} The CSMA distribution $p(\x)$ \eqref{eq_dist} can be expressed in the product form
%\begin{align*}
%p(\x)= \prod_{i \in V} f_i(x_i) \prod_{(i,j) \in E} f_{ij}(x_i,x_j), \; \; \x \in \{0,1\}^V,
%\end{align*}
%where the factor function $f_i(x_i)=\exp(v_i x_i)$, $f_{ij}(x_i,x_j)= \i(x_i+x_j\leq1)$. Note that the indicator functions $\i(x_i+x_j\leq1)$ ensure that only the independent sets of the conflict graph have non-zero probability. $r=\{X_1,X_2, f_1, f_2, f_{12}\}$ is a region with variables $X_1,X_2$, and factors $f_1,f_2,f_{12}$. 
%
%\textbf{Remark:} In this paper, we will deal with regions, in which if the variables in the region are known, the factors present in that region are implicitly understood. For the Example 2 considered above, one simple way to construct such regions is, given some set of variables $S \subset V$, include the factors $\{f_i\}_{i \in S}$, and $\{f_{ij}\}_{\{i,j \in S | (i,j) \in E \}}$. For example, consider a simple 4-cycle conflict graph as shown in Figure \ref{fig_ring}.  Then if we say the variables in a region are ${1,2}$, it will be understood that the region is given by $r=\{X_1,X_2, f_1, f_2, f_{12}\}$. For notational simplicity, unless we explicitly require,  we denote a region $r$ with the indices of the variables present in it. 


 
\emph{Regions and Counting numbers:} For a given conflict graph $G(V,E)$, let $\Re \subseteq 2^V$ denote some collection of subsets of the vertices $V$. These subsets are referred to as \emph{regions}. Further, assume that each region $r\in \Re$ is associated with an integer $c_r$ called the \emph{counting number} of that region. 
%$\{r \in \Re | i \in r\} \neq \Phi$
A valid set of regions $\Re$, and the corresponding counting numbers $\{c_r\}$ should satisfy the following two basic rules: a) Each vertex in $V$ should be covered in at least one of the regions in $\Re$, \ie, $\bigcup_{r \in \Re} r = V$, b) For every vertex, the counting numbers of all the regions containing it, should sum to $1$, \ie, 
\begin{align}
\sum_{\{r \in \Re | i \in r\}} c_r =1, \; \; \forall i \in V. \label{eq_counting_general} 
\end{align}

\emph{Regional schedule:} The regional schedule at a region $r \in \Re$, denoted by $\x_r \in \{0,1\}^{r}$, is defined as the set of variables corresponding to the transmission status of the vertices in that region, \ie, $\x_r:=\left\lbrace x_k \; | \; k \in r  \right\rbrace.$ Let $\I_r:= \{\x_r \; | \; x_i + x_j \leq 1, \forall  (i,j) \in E\}$ denote the set of feasible regional schedules. The schedules in $\I_r$ are said to be locally feasible at the region $r$.

\emph{Regional distribution and entropy:} If $b$ denotes the probability mass function of the random variable $\x = [x_i]_{i=1}^N$, then the regional distribution $b_r$ denotes the marginal distribution of $b$ corresponding to $\x_r \subset \x$. In the special case of a region being a singleton set, \ie, $r=\{i\}$ for some $i \in V$, then we denote the corresponding marginal distribution as $b_i$ instead of $b_{\{i\}}$.  The entropy $H_r(b_r):=  -\sum_{\x_r}b_r(\x_r) \ln b_r(\x_r)$ is called the regional entropy at the region $r$.

\emph{Local consistency:} Let $\{b_r\}_{r \in \Re}$ shortly denoted as $\{b_r\}$, be some set of regional distributions which may not necessarily correspond to valid marginals of any distribution $b$. If every two regions $r, q \in \Re$ such that $r \subset q$, satisfy $\sum_{\x_q \setminus x_{r}} b_q (\x_q) = b_r(\x_r)$, $\forall \x_r$, then the set of distributions $\{b_r\}$ are said to be locally consistent, and are referred to as pseudo marginals. 

%A \emph{Region graph} compactly captures these set of local consistency equations. Specifically, the set of regions $\Re$ constitute the vertices of the region graph, and two regions $r \subset q \in \Re$ share an edge if there does not exist any other region $s \in \Re$ such that $r \subset s \subset q$.  This condition for edges is useful in removing some redundant equations.

Now we use these definitions to introduce RFE. Assume that a valid collection of regions $\Re$, and the corresponding counting numbers are given.\footnote{We assume that all the singleton sets are present in the collection of the regions $\Re$. In case, this assumption is not satisfied, one can simply add those missing singleton sets with a counting number $0$.} Then the RFE for the CSMA distribution, with a fugacity vector $\v$,  is defined as follows. 
\begin{definition} (Regional Free Energy)
Let $\v$ be the fugacity vector of CSMA. Then, given a random variable $\x = [x_i]_{i=1}^N$ on the space of feasible schedules $\I$, and its probability distribution $b$, the RFE denoted by $F_{\Re}(b; \v)$ is defined as
\begin{align}
F_{\Re}(b; \v)= F_{\Re}(\{b_r\} ; \v) = U_{\Re}(\{b_r\}; \v) - H_{\Re}(\{b_r\}). \label{eq_RFE}
\end{align}
Here the first term, called the average energy, is given by the following weighted expectation
\begin{align}
U_{\Re}(\{b_r\}; \v)= - \sum_{r \in {\Re}}c_r \E_{b_r}\Big[\sum_{j \in r} v_j x_j\Big]. \label{eq_averageenergy}
\end{align}
The second term $H_{\Re}(\{b_r\})$, known as the \emph{Regional entropy}, is an approximation to the actual entropy $H(\x)$, and is given by
\begin{align}
H_{\Re}(\{b_r\})= \sum_{r \in {\Re}}c_r H_r (b_r). \label{eq_k_ent}
\end{align}
 \end{definition}

The stationary points\footnote{Here, constrained stationary point refers to a stationary point of the Lagrangian function of the RFE that enforces the local consistency contraints.}  of the RFE with respect to the regional distributions $\{b_r\}$, constrained over the set of psuedo marginals, provide accurate estimates \cite{book_martin} of the marginal distributions of $p(\x)$ in \eqref{eq_dist}. In other words, if the set of psuedo marginals $\{b^*_r\}$ is a stationary point of the RFE $F_{\Re}(\{b_r\} ; \v)$, then $\{b^*_r\}$ correspond to the estimates of the marginal distribution of $p(\x)$ over the respective regions. In particular, $b_i^*(x_i=1)$ provides an estimate of the service rate $s_i$  corresponding to the fugacity vector $\v$. 


%One of the major challenges in using this Kikuchi approximation framework for algorithm like CSMA is in choosing the regions in such a way that algorithm will retain the property of distributed implementation. Firstly, the generation of the regions themselves should be done in a distributed manner. Furthermore, any computations that you do to find the optimal regional distribution $\{b_r\}$ should have a distributed implementation. 
%With these trade-offs in consideration, we choose certain cliques of the interference graph as the regions. Firstly, the regions can be generated easily by using only the information on the local topology. More importantly, Kikuchi approximation can be significantly improved if the effect of short loops can be eliminated. Here, by choosing the maximal cliques as regions, the effect of triangles which form the smallest loop is completely eliminated. Hence, there is a significant improvement in the performance compared to Bethe approximation.

==> Arxiv TMC_journal/regions_choice.tex <==
\begin{figure}
\begin{center}
\begin{tikzpicture}[scale=.7]
\draw
    (1,0)--(0.30,0.95)
    (0.30,0.95)--(-0.80,0.58) 
    (-0.80,0.58)--(-0.80,-0.58)
    (-0.80,-0.58)--(0.30,-0.95)
    (0.30,-0.95)--(1,0);
    
    \fill (1,0) circle(0.06cm);
    \fill (0.30,0.95)circle(0.06cm);
    \fill (-0.80,0.58)circle(0.06cm);
    \fill (-0.80,-0.58)circle(0.06cm);
    \fill (0.30,-0.95)circle(0.06cm);
    
    \draw (2-6,-.9) -- (2-6,.9) -- (3.8-6,.9) -- (3.8-6,-.9) -- (2-6,-.9); 
    
    \fill (2-6,-.9) circle(0.06cm);
    \fill (2-6,.9)circle(0.06cm);
    \fill (3.8-6,.9)circle(0.06cm);
    \fill (3.8-6,-.9)circle(0.06cm);
    
%       \fill (2-6,-.9) circle(0.06cm);
%    \fill (2-6,.9)circle(0.06cm);
%    \fill (3.8-6,.9)circle(0.06cm);
%    \fill (3.8-6,-.9)circle(0.06cm);
    
\node at (2-6-.2,-.9) {\begin{scriptsize}3\end{scriptsize}};
\node at (2-6-.2,.9) {\begin{scriptsize}1\end{scriptsize}};
\node at (3.8-6+.2,.9) {\begin{scriptsize}2\end{scriptsize}};
\node at (3.8-6+.2,-.9) {\begin{scriptsize}4\end{scriptsize}};
%\node at (1,0) {\begin{scriptsize}5\end{scriptsize}};    
    
%    \fill (0.30,-0.95)circle(0.06cm);

\node at (-0.80-0.2,0.58) {\begin{scriptsize}1\end{scriptsize}};
\node at (0.30,0.95+.2) {\begin{scriptsize}2\end{scriptsize}};
\node at (-0.80-.2,-0.5) {\begin{scriptsize}5\end{scriptsize}};
\node at (0.30,-0.95-.2) {\begin{scriptsize}4\end{scriptsize}};
\node at (1+.2,0) {\begin{scriptsize}3\end{scriptsize}};
\end{tikzpicture}
\end{center}
\caption{Illustration of Ring topology: 4-cycle, 5-cycle.}
\label{fig_ring}
\end{figure}
\begin{figure*}
\begin{minipage}{.5 \textwidth}
\centering
\includegraphics[scale=0.5]{sq_two_pent_graph.pdf}
\caption{A typical realization of a random geometric graph that is generally used to model wireless networks. Here, each vertex represents a wireless link, and two vertices are connected if they are within a certain distance called the interference radius.}
\label{fig_typical}
\end{minipage}
\begin{minipage}{.5 \textwidth}
\includegraphics[scale=0.5]{Bethe_Ring_Absolute.pdf}
\caption{Bethe approximation error for cycles of different sizes}
\label{fig_cycle}
\end{minipage}
\end{figure*}
The accuracy of the Regional approximation crucially depends on the choice of the regions. As the collection of regions becomes larger, the accuracy improves. However, for arbitrary choices of regions, the computation of RAF may not be amenable to a distributed implementation. Hence, the major challenge in using the Regional approximation framework for an algorithm like CSMA, is in choosing the regions that are as large as possible, while retaining the property of distributed implementation. 
%With this requirement in consideration, we propose a property called the regional decomposition property which will guide us in the selection of regions.
%\begin{definition} (Regional decomposition property)
%Let $\Re$ a given collection of regions. If the Regional entropy maximization problem \eqref{eq_opt_step1} is equivalent to separately maximizing the regional entropy $H_r(b_r)$ at each region $r \in \Re$, then the collection $\Re$ is said to be regionally decomposable. In particular, the solution of \eqref{eq_opt_step1} should be equal to the solutions obtained by
%\begin{align}
% \underset{b_r}{\arg \max} & \; H_r(b_r), \; \; \text{subject to} \label{eq_opt_regional}\\
%\sum_{x_r : x_i=1} b_r (x_r) &= s_i, \; \; \; i \in r, \nonumber \\
% b_r(\x_r)&=0, \; \; \; \x_r \notin \I_r.  \nonumber
% \end{align}
%\end{definition} 
For example, if we consider a special case of Regional approximation called the Bethe approximation \cite{yedidia}, simple distributed algorithms are known for the fugacities \cite{bethe_jshin} \cite{allerton_bethe}.

\subsection{Bethe approximation}
Under the Bethe approximation framework \cite{yedidia}, the collection of regions $\Re$ includes only the regions of cardinality one and two. Specifically, those are the regions corresponding to the vertices, and the edges of the conflict graph. Hence, the Bethe approximation is easy to implement. However, its accuracy is poor for topologies that contain many small cycles. Hence, Bethe approximation is not the right choice for typical wireless networks that inherently contain small cycles. (For example, Figure \ref{fig_typical} shows a typical realization of a random geometric graph that is generally used to a model wireless network. It can be observed that Figure \ref{fig_typical} contains small cycles.)



We consider a ring topology (see Figure \ref{fig_ring}), and plot the percentage error due to the Bethe approximation \cite[Section III]{bethe_jshin} as a function of the cycle size in Figure \ref{fig_cycle}. Here, the Bethe approximation error is defined as the loss in service rate that occurs due to the approximation used in computing the fugacitites (precise definition is provided later).  It can be observed from Figure \ref{fig_cycle}, that the significant error is mainly due to cycles of size $3,4$. For cycles of size $5$ or more, the error is within $5$ percent. Hence, if we can include the cycles of size $3,4$ in the collection of regions, the error can be significantly improved. To that end, we discuss a class of Regional approximations called the Kikuchi approximations, which can accommodate the cycles in the collection of regions.


\subsection{Kikuchi approximation}
Kikuchi approximation is a special case of Regional approximation framework. The Kikuchi approximation framework imposes certain restrictions on how the regions, and the counting numbers can be selected. Specifically, 
\begin{enumerate}
\item The collection of regions $\Re$ should be closed under intersection.
\item The counting numbers should satisfy
\begin{align}
\sum_{\{q \in \Re \;|\; r \subseteq q\}} c_q =1, \forall r \in \Re. \label{eq_counting0}
\end{align}
\end{enumerate}
\emph{Remark:} It can be observed that the constraints \eqref{eq_counting_general} imposed by the general Regional approximation are weaker than the constraints \eqref{eq_counting0} imposed by the Kikuchi approximation. In particular, Regional approximation imposes the constraints \eqref{eq_counting0} only on the singleton regions, \ie,
\begin{align}
\sum_{\{q \in \Re \;|\; \{i\} \subseteq q\}} c_q =1, \forall i \in V.
\end{align}
Cluster Variation Method (CVM) \cite{yedidia} is a well-known approach to obtain a collection of regions $\Re$, that satisfy the properties of the Kikuchi approximation framework. In this approach, we start with an initial set of regions $\Re_0$ called the maximal regions. Then $\Re$ is obtained by including the set of the maximal regions $\Re_0$, and all the regions that can be obtained by taking all the possible intersections of the maximal regions. Further, the counting numbers are computed as follows. First, all the maximal regions are assigned a counting number $1$. Then the counting numbers of the other regions are iteratively computed using
\begin{align}
c_r = 1 - \sum_{\{q \in \Re \;|\; r \subset q\}} c_q, \; \; \forall r \in \Re. \label{eq_counting_formula}
\end{align}

In the next section, we use this Kikuchi approximation framework to the improve the approximation error incurred due to 3-cycles. 
%Specifically, we consider the Kikuchi approximation with the set of maximal cliques as $\Re_0$, and derive explicit formulas for the Region approximated fugacities.

==> Arxiv TMC_journal/sec_four_cycles.tex <==
In Section \ref{sec_clique}, we have considered clique based regions to improve the error due to 3-cycles. In this section, we focus on improving the error due to 4-cycles. 
%For this task, a naive application of the standard cluster variation method is not amenable to distributed implementation. We take advantage of the fact that our results Theorem \ref{thm_step1}, \ref{thm_step2} are applicable for arbitrary choice of regions, and propose an alternate method to select the regions which results in a distributed algorithm. 
%Specifically, in this \emph{4-cycle based approach}, in addition to the clique based regions, we also consider the 4-cycle regions\footnote{In this paper, we only deal with 4-cycles that do not have a chord. Whenever, we use the term 4-cycle, we mean a 4-cycle without a chord.} which do not have a chord within them (Figure \ref{fig_ring} shows a 4-cycle without a chord).
%\noindent \emph{Remark:} This collection of $\Re$ does not fall under the Kikuchi approximation framework since our $\Re$ may not include all the intersections of the 4-cycle regions. 
%
%\begin{itemize}
%\item All the 4-cycles\footnote{In this paper, we only deal with 4-cycles that do not have a chord. Whenever, we use the term 4-cycle, we mean a 4-cycle without a chord.} in the conflict graph.
%
%\item All the clique regions computed in the clique based approach (Algorithm 1).
%
%\item The regions corresponding to all the edges and the vertices of the conflict graph.
%\end{itemize}
%
%
%
%In particular, in this 4-cycle based approach the collection of regions $\Re$ includes
%\begin{itemize}
%\item All the 4-cycles\footnote{In this paper, we only deal with 4-cycles that do not have a chord. Whenever, we use the term 4-cycle, we mean a 4-cycle without a chord.} in the conflict graph
%\item All the cliques in the conflict graph
%\end{itemize}
%
%
Specifically, in this 4-cycle based approach, our collection of regions at a vertex $i$ includes
\begin{itemize}
\item All the 4-cycle regions that include vertex $i$.
\item All the cliques that include vertex $i$.
\end{itemize}
Further, the counting numbers are computed using \eqref{eq_counting_formula}. 

\emph{Remark:} In this paper, we only deal with 4-cycles that do not have a chord. Whenever, we use the term 4-cycle, we mean a 4-cycle without a chord.


Observe that the above collection of regions does not fall under the standard CVM framework, since our collection of regions may not include all the intersections of the 4-cycle regions.  The advantage of proposing this collection of regions is that it results in a distributed solution for fugacities. In particular, as we will prove in Theorem \ref{thm_4cycle}, the regional entropy maximization problem \eqref{eq_opt_step1} which is possibly a non-convex problem, decouples into local entropy maximization problems at each region. Further, these local entropy maximization problems have a closed form solution as stated in Theorem \ref{thm_grid_formula}. We now formally state these results.

%\begin{enumerate}
%\item Since the main goal is to improve the error due to 4-cycles and 3-cycles, we can safely ignore the intersections which do not result in these structures, and thereby reduce the complexity of our algorithm.
%
%\item This choice of regions lead to a distributed solution for fugacities. In particular, as we will prove in Theorem \ref{thm_4cycle}, the approximate entropy maximization problem \eqref{eq_opt_step1} which is possibly a non-convex problem, decouples into local entropy maximization problems at each region. Further, these local entropy maximization problems have a closed form solution as stated in Theorem \ref{thm_grid_formula}.
%\end{enumerate}



%This collection of $\Re$ does not fall under the Kikuchi approximation / Cluster variation method framework since our collection of regions may not include all the intersections of the 4-cycle regions. 

%\noindent \emph{Remarks:} 
%\begin{enumerate}
%\item This collection of $\Re$ does not fall under the Kikuchi approximation / Cluster variation method framework since our collection of regions may not include all the intersections of the 4-cycle regions. 
 
%\end{enumerate}
%The counting numbers are computed using \eqref{eq_counting_formula}. 



%In Section \ref{sec_clique}, we have considered clique based regions to improve the error due to 3-cycles. In this section, we focus on improving the error due to 4-cycles. In particular, as shown in Figure \ref{fig_ring}, we consider the 4-cycle regions which do not have a chord within them. 

%In this approach, the regions are obtained by starting with an initial collection $\Re_0$ that includes the 4-cycles and maximal cliques of the conflict graph. Then we obtain $\Re$ by using the cluster variation method. The counting numbers are computed according to \eqref{eq_counting_formula}.
%Now, in Theorem \ref{thm_4cycle}, we characterize the RAF under this approach. 

\begin{theorem} \label{thm_4cycle}
Let the set of all the 4-cycles, and all the cliques be denoted by $\Re_{4C}$, $\Re_{Cl}$ respectively. Let $\Re= \Re_{4C} \cup \Re_{Cl}$ be the collection of regions. Let $\{b_r^*\}$ be the solution of the regional entropy maximization problem \eqref{eq_opt_step1}. For the clique regions $r \in \Re_{Cl}$, $b_r^*$ is given by \eqref{eq_reg_dist}. For the 4-cycle regions $r \in \Re_{4C}$, $b_r^*$ is given by the solution of the following optimization problem:
\begin{align}
 &\underset{b_r}{\arg \max}  \; H_r(b_r), \; \; \text{subject to} \label{eq_opt_4cycles}\\
& b_r(\x_r) \geq 0, \; \x_r \in \I_r; \;\; \sum_{\x_r \in \I_r} b_r(\x_r) =1,\nonumber\\
&\sum_{\x_r \in \I_r : x_i=1} b_r (\x_r) = s_i, \; \; \; i \in r. \label{eq_const_4cycle}
 \end{align}
 \end{theorem}
 \begin{proof}
As obtained in the proof of Theorem \ref{thm_clique}, the regional distributions of the set of cliques $\{b_r^*\}_{r \in \Re_{Cl}}$ are explicitly determined by the service rates $\{s_i\}$ as shown in \eqref{eq_reg_dist}. Hence, in the objective of \eqref{eq_opt_step1}, the entropy terms corresponding to the cliques regions are completely determined by the service rates. In other words, the entropy terms corresponding to the 4-cycles are the only terms that are to be considered while maximizing the objective \eqref{eq_opt_step1}. Further, since no clique or another 4-cycle can be a super set of a 4-cycle, from \eqref{eq_counting_formula}, it can be observed that $c_r=1$ for all the 4-cycle regions $r \in \Re_{4C}$. Hence, the optimization problem \eqref{eq_opt_step1} can be effectively reduced to an optimization problem over $\{b_r\}_{4C}$ as follows:

\begin{align}
  \underset{\{b_r\}_{r \in \Re_{4C}}}{\arg \max}&  \sum_{r \in \Re_{4C}}  H_r(b_r), \; \; \; \text{s.t.} \label{eq_semi_local}\\
  b_r(\x_r) &\geq 0, \; \x_r \in \I_r; \;\; \sum_{\x_r \in \I_r} b_r(\x_r) =1, \; r \in \Re_{4C},\nonumber\\
\sum_{\x_q \setminus \x_{r}} b_q (x_q) &= b_r^*(\x_r), \; \; \x_r \in \I_r,  r \in \Re_{Cl}, q \in \Re_{4C}, \text{ s.t. } r \subset q. \label{eq_consistency_semi}
%\sum_{\x_q \setminus x_{r}} b_q (\x_q) &= b_r(\x_r), \; \; \x_r \in \I_r, \text{ and } r, q \in \Re \text{ s.t. } r \subset q. \label{eq_consistency} \\
 %b_r(\x_r)&=0, \; \; \; \x_r \notin \I_r, r \in \Re_{4C},  \nonumber
% b_i(1)&=s_i, \; \; \; i=1\dots N. \nonumber
\end{align}  


Now, let us look at the constraints of \eqref{eq_semi_local} involving $q \in \Re_{4C}$. It is easy to observe that for a given 4-cycle region (without a chord) $q \in \Re_{4C}$, the only possible subsets in the clique regions $r \in \Re_{Cl}$ are the regions corresponding to edges $\Re_{E}$, and singleton sets. 

Further, for any $r=\{i,j\} \in \Re_{E}$, the only feasible schedules are $\I_{\{i,j\}}=\{(0,0), (1,0), (0,1)\}$. Similarly, for a singleton region $r=\{i\}$, we have $\I_{i}=\{0,1\}$. From \eqref{eq_reg_dist}, we also know that $b^*_{\{i,j\}}(1,0)=s_i$, $b^*_{\{i,j\}}(0,1)=s_j$, and $b^*_i(1)=s_i$. Hence, the set of constraints in \eqref{eq_consistency_semi} for a given $q \in \Re_{4C}$ effectively reduces to
\begin{align}
\sum_{\x_q \in \I_q: x_i=1,x_j=0} b_q (\x_q) &= s_i, \; \; \{i,j\}\in \Re_{E}, \text{ s.t.} \{i,j\} \subset q,  \label{eq_mini1}\\
\sum_{\x_q \in \I_q: x_i=0,x_j=1} b_q (\x_q) &= s_j, \; \; \{i,j\}\in \Re_{E}, \text{ s.t.} \{i,j\} \subset q,  \label{eq_mini2}\\
\sum_{\x_q \in \I_q: x_i=1} b_q (\x_q) &= s_i, \; \; \forall i \in V, \text{ s.t. } \{i\} \subset q. \label{eq_mini3}
\end{align}
Note that we did not explicitly consider the constraints corresponding to $(0,0) \in \I_{\{i,j\}}$, $0 \in \I_{\{i\}}$, since they are implicitly captured by the normalization constraints in \eqref{eq_semi_local}.

For any feasible schedule of a 4-cycle region $\x_q \in \I_q$, by the definition of local feasibility, no more than one vertex across an edge can be active. Hence, for any $(i,j) \in E$ of the 4-cycle $q$, we have $\{\x_q \in \I_q | x_i=1, x_j=0\} = \{\x_q \in \I_q | x_i=1\}$. Hence, the constraints in \eqref{eq_mini1} - \eqref{eq_mini3} can be implicitly captured by \eqref{eq_mini3} alone.
Further, in \eqref{eq_semi_local}, there are no constraints that involve the optimization variables of different 4-cycle regions. Hence, the problem \eqref{eq_semi_local} decouples into independent optimization problem at each 4-cycle as given in \eqref{eq_opt_4cycles}.
\end{proof}
Now, we derive explicit formula for the solution of the optimization problem \eqref{eq_opt_4cycles}.
\begin{theorem} \label{thm_grid_formula}
Let $r \in \Re_{4C}$ be a 4-cycle region as shown in Figure \ref{fig_ring}. Then $b_r^*$, the solution of the optimization problem \eqref{eq_opt_4cycles} satisfies the expression \eqref{eq_loop_big} (displayed on the top of the next page).
\begin{figure*}[!t]
% ensure that we have normalsize text
\scriptsize
% Store the current equation number.
%\setcounter{MYtempeqncnt}{\value{equation}}
% Set the equation number to one less than the one
% desired for the first equation here.
% The value here will have to changed if equations
% are added or removed prior to the place these
% equations are referenced in the main text.
%\setcounter{equation}{5}
\begin{align}
\label{eq_loop_big}
\begin{split}
\frac{b_r^*(\x_r^1)}{b_r^*({\bf{0}})}&=\frac{\sqrt{(s_1 (s_2+s_3-s_4-1)+s_2 (s_3+s_4-1)+(s_3-1) (s_4-1))^2+4 s_1 s_4 (s_1+s_4-1) (s_2+s_3-1)}}{2 (s_1+s_2-1) (s_1+s_3-1)}\\
&\; \;\;+\frac{-2 s_1^2-s_1 (s_2+s_3+s_4-3)-s_2 s_3-s_2 s_4+s_2-s_3 s_4+s_3+s_4-1}{2 (s_1+s_2-1) (s_1+s_3-1)}.
\end{split}
\end{align}
% Restore the current equation number.
%\setcounter{equation}{\value{MYtempeqncnt}}
% IEEE uses as a separator
\hrulefill
% The spacer can be tweaked to stop underfull vboxes.
\vspace*{4pt}
\end{figure*}
In particular, if we assume homogeneous service rates, \ie, if $s_i=s,\; \forall i \in r$, then we have
\begin{align*}
\frac{b_r^*(\x_r^i)}{b_r^*({\bf{0}})}&=\frac{-1 + 4 s + \sqrt{1 - 4 s + 8 s^2}}{2 - 4 s}, \; \; \forall i \in r,
\end{align*}
where $\x_r^i$ denote the argument with $x_i=1, x_j=0, \forall j \in r\setminus \{i\}$, and ${\bf{0}}$ denote the argument with $x_j=0, \forall j \in r$.
\end{theorem}
\begin{proof}
We prove for the case of homogeneous service rates. The proof can be easily extended to the general case. It can be shown \cite[Section 3.5]{libin_book} that the solution of a maximum entropy problem of the form \eqref{eq_opt_4cycles} is given by a product form distribution
\begin{align}
b_r^*(\x_r)& = \frac{\prod_{i \in r} \lambda^{x_i}}{Z}, \; \; \x_r \in \I_r, \label{eq_prod_4cycle}
\end{align}
for some $\lambda >0$. Here $Z$ is the normalization constant. The parameter $\lambda$ should be obtained by using the feasibility constraints \eqref{eq_const_4cycle}. Further observe that the ratio 
\begin{align}
\frac{b_r^*(\x_r^i)}{b_r^*({\bf{0}})} = \lambda, \;\;\forall i \in r. \label{eq_ratio}
\end{align}
For the 4-cycle region in Figure \ref{fig_ring}, the feasible schedules consists of  a) four schedules in which only one vertex is active, b) two schedules in which only the diagonal vertices are active. Using this structure in  \eqref{eq_const_4cycle}, \eqref{eq_prod_4cycle} we obtain 
\begin{align}
s= \frac{\lambda^2 + \lambda}{1+ 2 \lambda^2 + 4 \lambda}. \label{eq_quadratic}
\end{align}
Solving the quadratic equation \eqref{eq_quadratic}, and using the observation \eqref{eq_ratio} gives the required result.
\end{proof}

\emph{Remark:} In Theorem \ref{thm_grid_formula}, we obtained a closed form expression for the regional distributions corresponding to 4-cycles. We already got closed form expressions for the regional distributions corresponding to cliques in \eqref{eq_reg_dist}. Hence, the RAF \eqref{eq_lf_gf} under our 4-cycle based approach can be explicitly computed without solving any optimization problems.


Now to demonstrate our 4-cycle based approach, we consider the widely studied grid topology \cite{marbach}, and derive the RAF explicitly. A $4 \times 4$ grid topology is illustrated in Figure \ref{fig_grid}.
\begin{cor}
Let $s_i=s,\; \forall i \in \N$ be the service rate requirements for a grid topology. Then the RAF under the 4-cycle based method is given by
\begin{align*}
\exp(\tilde{v}_i)&=
\begin{cases}
\frac{\left(-1 + 4 s + \sqrt{1 - 4 s + 8 s^2}\right)^4}{16 (1-s) s^3}, \; \; \text{ if } |\N_i|=4, \\
\frac{\left(-1 + 4 s + \sqrt{1 - 4 s + 8 s^2}\right)^2}{4 s ( 1-2s)}, \; \; \text{ if } |\N_i|=3, \\
\frac{-1 + 4 s + \sqrt{1 - 4 s + 8 s^2}}{2 - 4 s},    \; \; \text{ if } |\N_i|=2.
\end{cases}
\end{align*}
\end{cor}
\begin{proof}
We prove the result for a vertex of degree $4$. Other cases can be obtained similarly. Consider a vertex $i$ with degree 4 (for example, vertex 11 in Figure \ref{fig_grid}). Then the vertex $11$ belongs to four 4-cycle regions namely $\{7,8,11,12\},\{11,12,15,16\},\{6,7,10,11\},\{10,11,14,15\}$ . Each of these 4-cycle regions will have a counting number \eqref{eq_counting_formula} equal to $1$. Further, the intersection of these 4-cycle regions results in 4 edge based regions namely $\{11,7\},\{11,10\},\{11,15\},\{11,12\}$. Since each edge region has two super sets in the form of 4-cycles, the counting number \eqref{eq_counting_formula} of each of these edges is equal to $-1$. Further, the intersection of the edges result in the singleton set containing the considered vertex $11$. Since, all the four edges, and the four 4-cycles are super sets for this singleton vertex, the counting number of this singleton set  computed using \eqref{eq_counting_formula}  is equal to $1$. Now, from Theorems \ref{thm_4cycle}, \ref{thm_grid_formula}, we know the expressions for the optimal regional distributions $\{b_r^*\}$ of all the regions. Substituting these expressions in the formula for the RAF \eqref{eq_lf_gf} derived in Theorem \ref{thm_step2} gives the required result.
\end{proof}

\emph{Remark on Implementation:}
A vertex in the conflict graph requires the two hop neighbourhood topology to determine the 4-cycle regions that the vertex is involved in. This two hop topology can be obtained by using a simple broadcast scheme with the neighbours. For example, see \cite[Section VI-C]{bp_csma} for details.
%From the above example, it is clear that



==> Arxiv TMC_journal/subregion_algo.tex <==
\input{figure.tex}
We now propose a distributed algorithm to estimate the fugacities. Each link in the network can independently execute the algorithm once it obtains the a) target service rates of the neighbours, b) the local neighbourhood topology, \ie, which of its neighbours share an edge among themselves in the conflict graph. 


There are mainly two steps in the algorithm at a link $i$. The first step involves computing the maximal cliques\footnote{Note that, this overhead of computing the maximal cliques is involved in the I-GBP algorithm \cite{bp_csma} too.}, and their intersections in which the link $i$ is part of. The next step is to compute its fugacity by using the formula \eqref{eq_main}. We introduce some notations before we present the algorithm.

\emph{Notation:} Let $\Re_0^i$ be the collection of maximal cliques of the conflict graph $G(V,E)$ in which the vertex $i$ is part of. For example, if we consider the graph in Figure \ref{fig_cliq},  then $\Re_0^2 =\{\{1,2\}, \{2,8,7\}$, $\{2,3,7\}\}$. Similarly $\Re_0^3= \{\{2,3,7\}, \{3,5,6,7\}, \{3,4\} \}$. Using the information about the local topology, any standard algorithm like \cite{cliques_complexity} can be used for finding this set of maximal cliques $\Re_0^i$. For every maximal clique $r \in \Re_0^i$, let us associate a constant $c_r=1.$
\noindent\rule[0.5ex]{\linewidth}{0.5pt}
\textbf{Distributed algorithm at link $i$}\\
\noindent\rule[0.5ex]{\linewidth}{0.5pt}
\; \; \emph{Input:}  $\Re_0^i$, service rates $\{s_j\}_{j \in \N_i}$; \hspace{0.25cm}
\emph{Output:}  fugacity $\tilde{v}_i$.
\begin{enumerate}
\item Initialize $l=0$. 

\item Consider the set of all the intersections of the cliques in $\Re_l^i$ to obtain $\Re_{l+1}^i:= \{q_1 \cap q_2 \;|\;  q_1, q_2 \in \Re_{l}^i, q_1 \neq q_2\}.$ If  there are no intersections, \ie, $\Re_{l+1} = \Phi$, go to Step 6; Else continue.

\item From the set $\Re_{l+1}^i$, discard the cliques which are proper subsets of some other cliques in $\Re_{l+1}^{i}$, \ie, discard $r \in \Re_{l+1}^i$ if there exist any other set $q \in \Re_{l+1}^i$ such that $r \subset q$.



\item For each clique $r \in \Re_{l+1}^i$, compute 
\begin{align}
c_r= 1 - \sum_{q \in \S(r)} c_q, \label{eq_counting}
\end{align}
where $\S(r)=\{q \in \cup_{k \leq l}\Re^i_{k}\; | \; r \subset q\}$ is the set of cliques which are super sets of a given set $r$.
\item Increment $l$ by $1$, and go to step 2.

\item Let $\Re^i:= \cup_k \Re_k^i$ denote the collection of all the regions computed above. Then the fugacity is computed as
\begin{align}
\exp(\tilde{v}_i) = s_i \prod_{r \in {\Re^i}} \Big(1- \sum_{j \in r} s_j \Big)^{-c_r}.  \label{eq_main}
\end{align}
\end{enumerate}
\noindent\rule[0.5ex]{\linewidth}{0.5pt}
\emph{Complexity:} The worst case complexity incurred by a link to compute the corresponding maximal cliques $\Re_0^i$ is $O(3^{d/3})$, where $d$ is the the maximum degree of the graph \cite{cliques_complexity}. Hence, for spatial networks, where the degree of the graph does not scale with the network size, our algorithm computes the fugacities with $O(1)$ complexity. 

\emph{Information exchange:} The information exchange required for our algorithm is very limited, since the algorithm is fully distributed except for obtaining the local topology information and neighbours' service rates.

\emph{Simple example:} Let us consider the conflict graph shown in Figure \ref{fig_cliq}, and compute the fugacity for the link $2$ using the proposed algorithm. Then the set of maximal cliques containing the vertex $2$, will be $\Re_0^2 =\{\{1,2\}, \{2,8,7\}$, $\{2,3,7\}\}$. Considering their intersections we get $\Re_1^2=\{\{2,7\}, \{2\}\}$. However, we discard the set $\{2\}$ since it is a proper subset of $\{2,7\}$. Hence $\Re_1^2= \{\{2,7\}\}$. From \eqref{eq_counting}, it can be easily observed that for the set $\{2,7\}$, $c_r=-1$, since it has two super sets namely $q_1=\{2,8,7\}, \;q_2= \{2,3,7\}$  with $c_{q_1}=1, c_{q_2}=1$. As there are no further intersections to be taken in $\Re_1^2$, the following expression gives the fugacity $\exp(\tilde{v}_2)$:
\begin{align*}
\frac{s_2  (1-s_2-s_7)}{(1-s_1-s_2) (1-s_2-s_8-s_7) (1-s_2-s_3-s_7)}.
\end{align*}
Next, we prove that the Region approximated fugacities computed using the clique based approach are exact for a class of graphs called Chordal graphs.

==> Arxiv TMC_journal/sys_model.tex <==
We consider a single-hop wireless network with $N$ links. We use the letter $\N$ to denote the set of all the links in the network. We represent the network using the widely used conflict graph interference model ~\cite{libin, fast_mixing}. A conflict graph is an undirected graph $G(V,E)$, in which each vertex corresponds to a wireless link (Transmitter - Receiver pair), and two vertices share an edge if simultaneous transmissions from the corresponding wireless links result in a collision. For a given link $i \in V$, the neighbour set $\N_i := \{j : (i,j) \in E\}$ denotes the set of conflicting links. 

We consider a slotted time model, and use $\x(t)=[x_i(t)]_{i=1}^N \subseteq \{0,1\}^N$ to denote the transmission status (or \emph{schedule}) of the links in the network. Specifically,  if a link $i$ is scheduled to transmit in a given time slot $t$, then the link is said to be active, and $x_i(t)$ is set to $1$. We assume that an active link can transfer unit data in a given time slot, if none of its conflicting links are active in that slot. We define service rate of a link as the long-term fraction of time that the link is active.

\emph{Rate region:}  A schedule $\x$ is said to be \emph{feasible} if no conflicting links are active simultaneously. Hence, the set of feasible schedules is given by $\mathcal{I}:= \{\x \in \{0,1\}^N \; : \; x_i + x_j \leq 1, \; \forall (i,j) \in E\}$. Then the feasible rate region $\Lambda$, which is the set of all the possible service rates over the links, is the convex hull of $\I$ given by $\Lambda:= \{ \sum_{\x \in \I } \alpha_{\x} \x : \sum_{\x \in \I} \alpha_{\x}=1, \alpha_{\x} \geq 0, \forall \x \in \I \}.$  Next, we describe a basic CSMA algorithm~\cite{fast_mixing}.

\emph{Basic CSMA:} 
\label{subsec_acsma}
In this algorithm, each link $i$ is associated with a real-valued parameter $v_i \in \R$ (referred to as fugacity) which defines how aggressively a link captures the channel. In each time slot, one randomly selected link $i$ is allowed to update its schedule $x_i(t)$ based on the information in the previous slot:
\begin{itemize}
\item If the channel is sensed busy, \ie,  $\exists j \in \N_i$ such that $x_j(t-1)=1$, then $x_i(t)=0$.
\item Else,  $x_i(t)=1$ with probability $\frac{\exp(v_i)}{1+\exp(v_i)}$.
\end{itemize}
Except for the selected link $i$, all the other links do not update their schedule, \ie, $x_j(t)=x_j(t-1), \forall j \neq i$.
It can be shown that the above algorithm induces a Markov chain on the state space of feasible schedules. Further, the stationary distribution is a product-form Gibbs distribution \cite{fast_mixing} given by
%\begin{align}
%p(\x) =\begin{cases}
%\frac{1}{Z} \prod\limits_{  j  : x_j=1}\lambda_j , & \forall \x \in \mathcal{I}, \label{eq_dist} \\
%0,&\forall \x \in \{0,1\}^{\N} \setminus \mathcal{I},
%\end{cases}
%\end{align}
\begin{align}
p(\x)&= \frac{1}{Z(\v)} \exp\left(\sum_{i=1}^N x_i v_i\right), & \forall \x \in \I \subseteq \{0,1\}^N,  \label{eq_dist}
\end{align}
where $\v=[v_i]_{i=1}^N$, and $Z(\v)$ is the normalization constant. Then, due to the ergodicity of the Markov chain, the long-term service rate of a link $i$ denoted by $s_i$ is equal to the marginal probability that link $i$ is active, \ie, $p(x_i=1)$. Thus, the service rates and the fugacity vector $\v$ are related as follows:
\begin{align}
s_i&= p_i(1) = \sum\limits_{\x \in \I \; : \; x_i=1 } Z(\v)^{-1} \exp\left(\sum_{i=1}^N x_i v_i\right), \; \; \forall i \in \N, \label{eq_serv_fug}
\end{align}
where $p_i(1)$ denotes $p(x_i=1)$.


\emph{Problem Description:} The CSMA algorithm can support any service rate in the rate region if appropriate fugacities are used for the underlying Gibbs distribution \cite{libin}. We consider the scenario where the links know their target service rates, and address the problem of computing the corresponding fugacity vector. In principle, the fugacities can be obtained by solving the system of equations in \eqref{eq_serv_fug}.  Unfortunately, for large networks, solving these equations is highly intractable since it involves computing the normalization constant $Z(\v)$ which has exponentially many terms.  In this work, we propose simple, distributed algorithms to efficiently estimate the fugacities. Our solution is inspired by the well known Regional free approximation framework \cite{yedidia} which is reviewed in the next section. %It is worth nothing that Region-based approximation framework is generally useful in computing the service rates for given fugacities. The novelty of our work lies in using this framework to solve the reverse problem of computing the fugacities for a given service rate vector.

==> clique_algo.tex <==
We implement the following distributed algorithm at every node to determine maximal cliques that particular node is involved in.


\emph{Algorithm:}We assume that all the nodes are numbered in a centralized fashion and one hop exchange occurs through the network.So, we assume that each node has information about its neighbors and their neighbors i.e the node has information till 2-hop extent.Consider the algorithm at node $i$:
\begin{itemize}
\item Initially consider all the neighbors of $i$ as unmarked.
\item Select an unmarked neighbor $j$ and add it to a new list.
\item Now consider all the neighbors one by one and each time check if this neighbor of $i$ is also a neighbor to all the nodes in the above list.
\item When done with all the neighbors of $i$,we get a list of nodes which belong to a clique.Change the status of all the nodes in this list as marked.
\item If there exists an unmarked neighbor of $i$ go back to step 2 to and proceed by selecting one of unmarked neighbor.Else exit form the algorithm.
\end{itemize}
At the end of this algorithm we will have several lists of nodes,each of which is a clique involving node $i$.The clique involving maximum number of nodes will be maximal clique(s) involving node $i$.


Let us illustrate the algorithm above for node $2$ and node $3$ of conflict graph in \ref{fig_cliq}.Considering node $2$,since we assume that it has knowledge of it's 2-hop network,we have neighbors as $\N_2=\{1,8,7,3\}$ and their neighbors as $\N_1=\{2\}$ , $\N_8=\{2,7\}$, $\N_7=\{8,2,3,5,6\}$ and  $\N_3=\{2,4,5,6,7\}$.Initially let all the neighbors of $2$ be unmarked. Let us select an unmarked node $1$.We add this to a new list resulting in $\{1\}$. Now,checking if other neighbors of $2$ are neighbors of nodes in list.We do not have any such nodes.So,we have one list as $\{1\}$ .So mark $1$ in neighbors list. Now select another unmarked node $8$ and add to new list resulting in $\{8\}$.Checking with other neighbors,we can add $7$ to list because it is in neighbor list and is also a neighbor to node $8$ which makes the list $\{8,7\}$.we mark nodes $8$ and $7$ also. Now considering unmarked nodes,we have node $3$.Add it to new list to get $\{3\}$.Now check for other neighbors and we get that node $7$ can be added to list making it $\{3,7\}$.With this we mark node $3$.Now on checking we see that there are no unmarked neighboring nodes.So we stop and check all the lists obtained which are $\{1\}$,$\{8,7\}$ and $\{3,7\}$.Among these two lists have same maximum length of two because of which both contribute to maximal cliques.So,we have maximal cliques at node $2$ as $\{2,8,7\}$ and $\{2,3,7\}$.
Let us also do this for node $3$.We have neighbors as $\N_3=\{2,4,5,6,7\}$ and their neighbors as $\N_2=\{1,3,7,8\}$ , $\N_4=\{3\}$, $\N_5=\{3,6,7\}$, $\N_6=\{3,5,7\}$ and $\N_7=\{2,3,5,6,8\}$.Initially let all the neighbors of $3$ be unmarked. Let us select an unmarked node $2$.We add this to a new list resulting in $\{2\}$. Now,checking if other neighbors of $2$ are neighbors of nodes in list. We have node $7$ which is added to list. So,we have one list as $\{2,7\}$ .So mark $2$ and $7$ in neighbors list. Now select another unmarked node $4$ and add to new list resulting in $\{4\}$.Checking with other neighbors,we can do not have any nodes to add to list because no neighbor of node $3$ in neighbor of node $4$ which makes the list only $\{4\}$.we mark node $4$ also. Now considering unmarked nodes,we have node $5$.Add it to new list to get $\{5\}$.Now check for other neighbors and we get that node $6$ can be added to list making it $\{5,6\}$.We also notice that node $7$ can also be added to list because node $7$ is neighbor of both node $5$ and $6$ which makes the list $\{5,6,7\}$.With this we mark nodes $5$ and $6$.Now on checking we see that there are no unmarked neighboring nodes.So we stop and check all the lists obtained which are $\{2,7\}$,$\{4\}$ and $\{5,6,7\}$.Among these only one list has maximum length of three because of which it contributes to maximal clique.So,we have maximal clique at node $3$ as $\{3,5,6,7\}$.Visually we can see that the maximal cliques obtained from distributed algorithm are correct.

==> fug_comp.tex <==
Now, we could use results obtained from optimizing Kikuchi free energy function and locally compute fugacities at each node. 
Consider a node $i$. Till this point, we have information about all the regions at various levels of which node $i$ is part of. We also have computed $c_R$ for every region. We can now compute approximate global fugacities locally at this node using the formula as follows:
\noindent\rule[0.5ex]{\linewidth}{0.5pt}
\textbf{Fugacity at node $i$}\\
\noindent\rule[0.5ex]{\linewidth}{0.5pt}
\; \; \emph{Input:} $\{R,c_R\}$; \hspace{0.25cm}
\emph{Output:} $\lt_i$.
The optimal fugacity at node $i$ is given by as
\begin{align}
\lt_i =  \prod_{r \in {R}} \left(\frac{b_r(i=1)}{b_r(i=0)}\right)^{c_r} .  \label{eqn_imp}
\end{align}
where for every region $r$ from ${R}$, 
we have $b_r(i=1)$ as joint probability of region where all the nodes of region are in off/0 state while node $i$ is active. Since the region is clique ,we have
\begin{align}
b_r(i=1) = b_i . \label{side_1}
\end{align}
where $b_i$ is service rate of node $i$.
And we have $b_r(i=0)$ as joint probability of region where all the nodes of region are in off/0 state. Since the region is clique ,we have
\begin{align}
b_r(i=0) = 1 - \sum_{k \in r} b_k . \label{side_2}
\end{align}
where for every node $k$ belonging to the region $r$ we have $b_k$ as service rate of node $k$.
While $c_r$ is the $c_R$ value of region $r$.
\noindent\rule[0.5ex]{\linewidth}{0.5pt}

==> fug_proof.tex <==
In this section, we state our main theorem which explains the connection between our distributed algorithm for the fugacities, and the Kikuchi approximation. Recall that $\Re^i$ is the set of cliques computed in the distributed algorithm at link $i$. Then, it can be easily verified that the set of regions given by $\Re:= \cup_{i=1}^N \Re^i$, with $\{c_r\}$ computed in \eqref{eq_counting}, constitute a valid collection of Kikuchi regions\footnote{In fact, the regions computed in this paper are inspired by the cluster variation method \cite{yedidia}, which is a standard algorithm to generate valid regions.}, and counting numbers. 
%Further, the set of local consistency conditions can be captured using a region graph with the cliques in $\Re$ as its vertices. For example, Figure \ref{fig_reg} shows the region graph corresponding to the conflict graph considered in Figure \ref{fig_cliq}.

\begin{comment}
\begin{figure}
\centering
\includegraphics[scale=0.45]{regions.png} 
%\includegraphics[scale=0.31]{random_graph_new.eps} 
\caption{Region graph for conflict graph shown in Figure \ref{fig_cliq}}
\label{fig_reg}
\end{figure}
\end{comment}

The non trivial step of our algorithm is the formula \eqref{eq_main} proposed for the fugacities. The following theorem justifies the proposed formula. If CSMA algorithm employs the set of fugacities $\{\tilde{v}_i\}_{i=1}^N$ estimated in \eqref{eq_main}, then the service rates obtained by the CSMA, are close to the desired service rates. This is because, the desired service rates correspond to stationary point of the KFE defined by $\{\tilde{v}_i\}_{i=1}^N$ as stated below.
\begin{theorem} \label{thm_main}
Let $\tilde{\v}$ be a set of fugacities that define the Kikuchi free energy $F_K(\{b_r\}; \tilde{\v})$. A locally consistent set of pseudo marginals $\{b_r\}$ will be a stationary point of the KFE if and only if $\sum_{j \in r} b_j(1) < 1, \forall r \in \Re$, and
%\begin{align*}
%\exp(\vt_i)= \prod_{r \in \Re^i}\left(\frac{b_i(x_i=1)}{1-\sum_{j \in {r}}b_j(x_j=1)}\right)^{c_r}, \; \forall i
%\end{align*}
\begin{align}
\exp(\vt_i)= b_i(1) \prod_{r \in \Re^i}\Big(1-\sum_{j \in {r}}b_j(1)\Big)^{-c_r}, \; \forall i, \label{eq_thm}
\end{align}
where $b_i(x_i), b_j(x_j)$ are the regional distributions corresponding to the singleton region sets $\{i\}, \{j\}$ respectively.
\end{theorem}
\begin{proof}
Recall that a schedule $\x=\{x_i\}$ is feasible iff no two adjacent links of the conflict graph transmit simultaneously. Since all our regions are cliques of the conflict graph, for any feasible distribution that is locally consistent, we have  
\begin{align}
b_r(x_r)=
\begin{cases}
      b_j(1),  &\text{if } x_j=1, x_k=0, \forall k \in r\setminus \{j\},  \\
      1- \sum_{j \in r} b_j(1),  &\text{if } x_j=0, \forall j \in r, \\
      0,  &\text{otherwise}. \label{eq_reg_dist}
\end{cases}
\end{align}
An interesting implication of the above observation is, the KFE $F_k(\{b_r\}; \tilde{\v})$ in \eqref{eq_kfe}, which is in general a function of all the pseudo marginals, can now be expressed as a function of the singleton marginals alone. Specifically, the average energy is
\begin{align*}
U_K(\{b_r\}; \tilde{\v})&= - \sum_{r \in {\Re}} c_r \E_{b_r}\Big[\sum_{j \in r} \vt_j x_j\Big], \\
&= - \sum_{r \in {\Re}} c_r \Big( \sum_{j \in r} \vt_j b_j(1)  \Big), \\
&= -\sum_{j=1}^N \Big(\sum_{\{r \;|\; j \in r\}} c_r \Big) \vt_j b_j(1) = -\sum_{j=1}^N \vt_j b_j(1).
\end{align*}
Similarly, the term corresponding to a region $r$ in the Kikuchi entropy $H_K(\{b_r\})$ defined in \eqref{eq_k_ent} can be expressed as
\begin{align*}
&\sum_{x_r}b_r(x_r)\log b_r(x_r) \\
&= \Big(1-\sum_{j \in {r}}b_j(1)\Big)\log\Big(1-\sum_{j \in {r}} b_j(1)\Big) + \sum_{j \in {r}}b_j(1) \log b_j(1).
\end{align*}
Using this expression, the gradient of the Kikuchi free energy $F_K(\{b_j(1)\}; \tilde{\v})$ can be computed as
\begin{align*}
\frac{\partial F_K}{\partial b_i(1)} 
&= -\vt_i + \sum_{\{r | i \in r\}}c_r\Big(\log b_i(1) - \log\big(1-\sum_{j\in {r}}b_j(1)\big)\Big).
\end{align*}
By using the fact that $\sum_{\{r \in \Re | i \in r\}} c_r =1$, and setting the gradient to zero, the proof is complete.
\end{proof}

Next, we state a corollary of Theorem \ref{thm_main} which derives the fugacities that correspond to the Bethe approximation framework used in \cite{bethe_jshin}. Specifically, if the collection of regions $\Re$ is formed using only the edges and the vertices of the conflict graph, it results in the Bethe approximation framework.
\begin{cor}
For a given set of required service rates, the estimate of the fugacities $\{v_i^B\}$ obtained using the Bethe approximation framework is given by
\begin{align*}
\exp(v_i^B)= \frac{s_i (1-s_i)^{d_i-1}}{\prod_{j \in \N_i} (1-s_i-s_j)}, \; \forall i,
\end{align*}
where the set $\N_i$ denotes the neighbours of the vertex $i$ in the conflict graph, and the $d_i$ denotes the degree.
\end{cor}
\begin{proof}
The proof follows by observing a set of valid counting numbers for the regions. Specifically, the counting number of the regions corresponding to each edge in the conflict graph can be set to $1$, and the counting number of a region corresponding to a vertex can be set to $1-d_i$. Then using \eqref{eq_thm}, the proof is completed.
\end{proof}


%While it is easy to argue that the claim is true, it also follows from the fact that our distributed algorithm for computing the regions is inspired by a standard approach called cluster variation method \cite{book_martin} that is generally used to generate valid Kikuchi regions.


%\begin{theorem} \label{thm_kikuchi_free}
%Let $\{\vt_i\}_{i=1}^N$ be the fugacities estimated using \eqref{eq_main}. Then we get that the given service rates $\{s_i\}_{i=1}^N$ are obtained as stationary point for optimizing corresponding free energy function.
%\end{theorem}
%\begin{proof}
%
%Now,we consider the second part of kikuchi free energy. For every region we compute the term $\sum_{x_r}b_r(x_r)\log b_r(x_r)$. Since every region in kikuchi approximation is of clique form we have a generalized form.
%We have, 
%\begin{align}
%\sum_{x_r}b_r(x_r)\log b_r(x_r) = \sum_{i \in {r}}b_i\log(b_i) + (1-\sum_{i \in {r}}b_i)\log(1-\sum_{i \in {r}}b_i)	\label{eqn_proof_right}
%\end{align}
%When we consider the whole kikuchi free energy function we will have term from \eqref{egn_proof_left} and for each region we have term from \eqref{eqn_proof_right}. To optimize the free energy we partially differentiate free energy with service rate of each node as variable and set differentials to $0$.
%Consider a node $i$. When we partially differentiate free energy with respect to service rate $b_i$ of node $i$, term from \eqref{egn_proof_left} gives
%\begin{align}
%\frac{\partial}{\partial b_i} \Big[ -\sum_{i \in {V}}b_im_i  \Big] = -m_i \label{eqn_final_left}
%\end{align}
%Now, when term from \eqref{eqn_proof_right} for region $r$ is partially differentiated with $b_i$, it gives $0$ if region does not contain node $i$. If region contains node $i$, then we get two terms containing $b_i$ which get affected by differentiation.
%We Know,
%\begin{align}
%\frac{\partial}{\partial b_i} \Big[ x\log(x) \Big] = 1+\log(x) \label{eqn_diff_log1}
%\end{align}
%\begin{align}
%\frac{\partial}{\partial b_i} \Big[ (1-x
%)\log(1-x) \Big] = -1-\log(1-x) \label{eqn_diff_log2}
%\end{align}
%So,from \eqref{eqn_diff_log1} and \eqref{eqn_diff_log2} we get 2 terms from each region containing node $i$ which are $\log(b_i)$ and $-\log(1-\sum_{i \in {r}}b_i)$ which get multiplied by $c_r$.
%On a whole we get,
%\begin{align}
%-m_i+ \sum_{r \in {R}}c_r\left(\log(b_i)-\log(1-\sum_{i \in {r}}b_i)\right)=0
%\end{align}
%which can be written as
%\begin{align}
%-m_i+ \sum_{r \in {R}}\log\left(\frac{b_i}{1-\sum_{i \in {r}}b_i}\right)^{c_r}=0
%\end{align}
%If $\lt_i$ is introduced,we get
%\begin{align}
%\lt_i = \prod_{r \in {R}}\left(\frac{b_i}{1-\sum_{i \in {r}}b_i}\right)^{c_r}
%\end{align}
%which is same as
%\begin{align}
%\lt_i =  \prod_{r \in {R}} \left(\frac{b_r(i=1)}{b_r(i=0)}\right)^{c_r}
%\label{eqn_proof_fin}
%\end{align}
%This way we get many equations when free energy is partially differentiated with respect to all the nodes of network.These equations turn out to be the same approximate expressions used to compute fugacities $\{\lt\}_{i=1}^N$.
%Thus we prove that such approximately computed fugacities optimize kikuchi free energy for given set of service rates $\{s_i\}_{i=1}^N$.
%\end{proof}

==> model.tex <==
\begin{figure}[h]
\centering
\includegraphics[scale=0.45]{exampl.png} 
%\includegraphics[scale=0.31]{random_graph_new.eps} 
\caption{Example of a small conflict graph consisting of 7 labeled nodes .}
\label{fig_cliq}
\end{figure}
Consider single hop wireless network model as shown in \eqref{fig_cliq}.We consider conflict graph pair wise model where we assume that adjacent nodes cannot transmit together. We want compute fugacities of all the nodes $\{\lt\}_{i=1}^N$ given their service rates $\{s_i\}_{i=1}^N$. We use kikuchi approximation to construct region graph. We use these regions and formulate kikuchi free energy function which can be optimized to obtain approximate set of fugacities for which we achieve service rates.
In kikuchi approach,we begin with an initial set of regions $\{R_0\}$ such that every node $i$ in the network graph is included in atleast one region $r\in{\{R_0\}}$.
 We also make sure that there does not exist a region $r^1$ such that it is subregion of another region $r$ at same level. $$r^1\not\subseteq{r}$$. If there exists such region $r^1$ then it is discarded from $\{R_0\}$. For determination of initial set of regions $\{R_0\}$ with above constraints we have proposed a distributed algorithm which considers maximal cliques as constituents of $\{R_0\}$. We then construct set of regions $\{R_1\}$ by forming all possible intersections of regions in $\{R_0\}$. We make sure no two regions at this level are subregions to one other. This way for construction of set of regions $\{R_2\}$ we take intersections of regions from $\{R_1\}$. We keep doing this to construct regions at different levels till we reach a stage where we cannot go to next level because of no intersections between regions in that level. Finally we obtain a whole set of kikuchi regions $R=\bigcup\limits_{i}R_i$. 
Now we define counting numbers $c_R$ for all the regions in $\{R\}$. For a region $r$ we have counting number $c_r$ as $$c_r=1-\sum_{s\in{S(r)}}c_s$$ where $S(r)$ is set of all regions which are super-regions of region $r$ and belong to $\{R\}$. Counting number ensures that when all the regions are considered together each node effectively accounts only for once.
Let us consider graph in \eqref{fig_cliq} to compute kikuchi regions. For $\{R_0\}$ we consider maximal cliques in the graph which give regions as $\{1,2\}$,$\{2,3,7\}$,$\{2,7,8\}$,$\{3,5,6,7\}$ and $\{3,4\}$. These form $\{R_0\}$. Now we consider their intersections to get $\{R_1\}$. We get intersections like $\{2,7\}$,.. but we also get intersections like $\{2\}$ which are sub-regions of other regions so will be discarded. Finally, we get $\{R_1\}$ regions as $\{2,7\}$ and $\{3,7\}$. Now, we go for $\{R_2\}$ which has only one region $\{7\}$. We cannot go ahead because of no intersections between regions in $\{R_2\}$. Thus we have $R=R_0\cup{R_1\cup{R_2}}$ as illustrated in \eqref{fig_reg} where regions are linked to show dependency. Now, we compute counting numbers $c_R$. For regions in $\{R_0\}$ we have $c_R$ as $1$ because regions in $\{R_0\}$ don not have any super-regions. Then for region $\{2,7\}$ we have $c_R = 1-(1+1) = -1$ since region $\{2,7\}$ has two super-regions from $\{R_0\}$. Similarly,for region $\{3,7\}$ we have $c_R = 1-(1+1) = -1$. For region $\{7\}$ we have $c_R = 1-(1+1+1-1-1) = 0$ as region $\{7\}$ has three super-regions from $\{R_0\}$ and two super-regions from $\{R_1\}$. Now,we have regions $\{R\}$ and their counting numbers $\{c_R\}$.

\begin{figure}[h]
\centering
\includegraphics[scale=0.45]{regions.png} 
%\includegraphics[scale=0.31]{random_graph_new.eps} 
\caption{Region graph level wise for conflict graph in Fig.1}
\label{fig_reg}
\end{figure}

Considering free energy equation for kikuchi regions with counting numbers, we have 
\begin{align}
F=\sum_{r\in{R}}U_r-H_r
\label{eqn_energy_1}
\end{align}
where $U_r$ and $H_r$ are energy and entropy functions for a region $r$ which are given by
\begin{align}
U_r=\sum_{r \in {R}}c_r\sum_{x_r}b_r(x_r)E_r(x_r)
\label{eqn_energy_2}
\end{align}
and
\begin{align}
H_r=-\sum_{r \in {R}}c_r{x_r}b_r(x_r)log b_r(x_r)
\label{eqn_energy_3}
\end{align}
Using \eqref{eqn_energy_2} and \eqref{eqn_energy_3} in \eqref{eqn_energy_1},we have kikuchi free energy as
\begin{align}
F_K= \sum_{r \in {R}}c_r\left( \sum_{x_r}b_r(x_r)E_r(x_r) + \sum_{x_r}b_r(x_r)log b_r(x_r)\right)
\label{eqn_energy_4}
\end{align}

==> neighbourhood.tex <==
In this section, we propose a region-based approximation that improves the error beyond the clique-based approach, without explicitly using the information about the two-hop neighbours. The key idea is to use the fact that our results derived in Theorem \ref{thm_step1}, \ref{thm_step2} hold for any collection of regions, and go beyond the standard Kikuchi approximation / Cluster variation method based regions. Specifically, our collection of regions $\Re$ includes
\begin{itemize}
\item For each vertex, $i \in V$, we include a neighbourhood region $r=\N_i$.
\item All the clique based regions.
\end{itemize}
The counting numbers are computed using \eqref{eq_counting_formula}.

\noindent \emph{Remark:} This collection of $\Re$ does not fall under the Kikuchi approximation framework since our $\Re$ may not include the intersections of the neighbourhood regions.

Let $\Re_N$ denote the set of all the neighbourhood regions, and $\Re_C$ denote the set of all the clique regions in $\Re$. In the following theorem we show that the optimization problem \eqref{eq_opt_step1} decouples into local optimization problems at each neighbourhood.
\begin{theorem}
Let the collection of regions $\Re$ include the neighbourhood regions $\Re_{N}$, and all the clique regions $\Re_{C}$. Let $\{s_i\}$ be the required service rates. Let $\{b_r\}$ be the solution of the optimization problem \eqref{eq_opt_step1}. For any $r \in \Re_{C}$, the corresponding regional distribution $b_r^*$  is given by \eqref{eq_reg_dist}. For any $r \in \Re_N$, the corresponding $b_r^*$ is given by the following optimization problem:
\begin{align}
 \underset{b_r}{\arg \max} & \; H_r(b_r), \; \; \text{subject to} \label{eq_opt_neigh}\\
\sum_{x_r \in \I_r : x_i=1} b_r (x_r) &= s_i, \; \; \; i \in r.
 \end{align}
\end{theorem}
\begin{proof}
As discussed in Theorem \ref{thm_clique}, the regional $b_r^*$ of a clique are explicitly determined by the service rates. Further, 
\end{proof}

==> preliminaries.tex <==
\subsection{Product form distribution}
Let $S$ be a finite set, and let $X_i, i=1, 2, \dots, N$, be random variables each taking values in $S$. The joint PMF (probability mass function) of the random variables is succinctly denoted as $p(\x)$, where $\x=\{x_1,x_2, \dots, x_N \}$. Suppose that $p(\x)$ factors into a product of $M$ functions and is given by,
\begin{align}
p(\x)&= \frac{1}{Z} \prod\limits_{j=1}^M f_j(\x_j), \hspace{0.7cm} \x \in S^N.  \label{eq_factors}
\end{align}
The function $f_j(\cdot)$ has arguments $\x_j$ that are some non-empty subset of $\{x_1,x_2, \dots, x_N \}$. Here $Z$ is a normalization constant. Further, the product form distributions are generally represented using a graph called factor graph \cite{book_martin} that has two sets of nodes namely variable nodes and factor nodes corresponding to the variables and the functions in \eqref{eq_factors} respectively. An edge is drawn between a variable node and a factor node if the variable is an argument of that factor function.
\begin{comment}
\textbf{Factor graph:}
A factor graph \cite{yedidia} is a bipartite graph used to visualize the factorization structure of the joint distribution \eqref{eq_factors}. The factor graph has two sets of nodes called the \emph{variable nodes} and the \emph{factor nodes} corresponding to the variables and the functions in \eqref{eq_factors} respectively. The variable nodes are represented using circles while the factor nodes are represented using squares. An edge is drawn between a variable node and a factor node if the variable is an argument of that factor function.
  Let us now consider an example.\\
\begin{figure}
{
\begin{center}
\begin{tikzpicture}[scale=0.3]
%\draw (0,0) -- (-2,0.7);
%\draw (-2,-0.7) -- (0,0);
\draw (0,0) -- (0.7,0);
\draw (0.7,0) -- (0.7,0.7);
\draw (0.7,0.7) -- (0,0.7);
\draw (0,0.7) -- (0,0);
\node at (0.35,-0.7) {{$f_1$}};

\draw (2,0) -- (2.7,0);
\draw (2.7,0) -- (2.7,0.7);
\draw (2.7,0.7) -- (2,0.7);
\draw (2,0.7) -- (2,0);
\node at (2.35,-0.7) {{$f_2$}};

\draw (4,0) -- (4.7,0);
\draw (4.7,0) -- (4.7,0.7);
\draw (4.7,0.7) -- (4,0.7);
\draw (4,0.7) -- (4,0);
\node at (4.35,-0.7) {{$f_3$}};


\draw (-1.5,3)circle(0.4cm);
\node at (-1.5,4) {{$x_1$}};
\draw (0.5,3)circle(0.4cm);
\node at (0.5,4) {{$x_2$}};
\draw (2.5,3)circle(0.4cm);
\node at (2.5,4) {{$x_3$}};
\draw (4.5,3)circle(0.4cm);
\node at (4.5,4) {{$x_4$}};
\draw (6.5,3)circle(0.4cm);
\node at (6.5,4) {{$x_5$}};
%\node at (3,0.85+0.2) {$2$};





\draw (0.35,0.7) -- (-1.5,3-0.4); %A- x1
\draw (0.35,0.7) -- (0.5,3-0.4); %A- x2
\draw (0.35,0.7) -- (6.5,3-0.4); %A- x5

\draw (2.35,0.7) -- (0.5,3-0.4); %B- x2
\draw (2.35,0.7) -- (4.5,3-0.4); %B- x4

%\draw (4.35,0.7) -- (-1.5,3-0.4); %C- x1
\draw (4.35,0.7) -- (2.5,3-0.4); %C- x3
\draw (4.35,0.7) -- (6.5,3-0.4); %C- x5
\end{tikzpicture}
\end{center}
}
\vspace{-0.6cm}
\caption{Factor graph}
\label{fig_fg}
\end{figure}
\emph{Example} (A simple factor graph): Consider a simple distribution of the form
\begin{align*}
p(x_1,x_2,x_3,x_4,x_5)&= \frac{1}{Z} f_1(x_1, x_2 , x_5) f_2(x_2, x_4) f_3(x_3, x_5).
\end{align*}
Using the notation in \eqref{eq_factors}, the distribution can be succinctly represented as
\begin{align*}
p(\x)&= \frac{1}{Z} f_1(\x_1) f_2(\x_2) f_3(\x_3), 
\end{align*}
where, $\x=\{x_1, x_2, x_3, x_4, x_5 \}$, $\x_1=\{x_1, x_2,  x_5 \}$, $\x_2=\{ x_2,  x_4 \}$, $\x_3=\{x_3,  x_5 \}$. The factor graph corresponding to this example is shown in Figure \ref{fig_fg}.\\
\end{comment}
For the product form distribution considered in \eqref{eq_factors}, we are interested in the marginal probabilities called variable marginals and factor marginals.

\noindent \emph{Variable node marginals: }
The marginal probability distribution $p_i({x_i})$ corresponding to a variable node $i$, is obtained by summing $p(\x)$ over the variables corresponding to all other variable nodes, \ie, $p_i({x_i})= \sum_{\x \setminus x_i} p(\x)$, $x_i \in S$, $ i=1,\dots, N.$

\noindent \emph{Factor node marginals:} Corresponding to each factor node, $j=1, \dots, M$, the marginal probability function $\p_j({{\x}_j})$,  is obtained by summing $p(\x)$ over all the variables in $\x \setminus {\x}_j$. Let $N_j$ denote the number of arguments in $f_j$, \ie, $N_j= |\x_j|$. Then, 
$
\p_{j}({{\x}_j}) = \sum_{\x \setminus {\x}_j} p(\x)$, ${\x}_j \in S^{N_j}.$

Let $\pv:=\{p_i\}_{i=1}^N$, $\pn:=\{\p_j\}_{j=1}^M$ denote the collection of all the variable node marginals and  the factor node marginals corresponding to the distribution $p(\x)$ respectively. Next, we discuss the Bethe approximation \cite{book_martin} which is used to estimate these marginal probability distributions.
\subsection{Bethe approximation}
%One approach to computing the partition function corresponding to the distribution $p(\x)$,  is to minimize a function called Gibbs free energy (GFE) over all the valid probability distributions on the state space $S^N$. However, as $N$ becomes large, even this procedure is intractable, as the optimization variables take exponentially large memory to store. We hence take recourse to the Bethe approximation, which is an approximate, but a more practical technique to estimate the marginals explicitly \cite{yedidia} . Next, we introduce the concepts of Bethe free energy and Bethe optimization with focus on the application for CSMA networks. 
\subsubsection{Bethe free energy (BFE)}
Consider a probability distribution $p(\x)$ of the form \eqref{eq_factors} for which we are interested in finding the marginals. Let $b(\x)$ be some distribution on $S^N$, whose factor and variable marginals are given by $\bn=\{\b_j\}_{j=1}^M$ and $\bv=\{b_i\}_{i=1}^N$. Here, $p(\x)$ is referred to as the \emph{true} distribution, and $b(\x)$ is referred to as the \emph{trial} distribution as it is used to estimate the true distribution $p(\x)$. Next, we define the Bethe entropy, which is required for the definition of BFE. The Bethe entropy of a distribution $b(\x)$ is a weighted sum of the entropies corresponding to the factor and the variable marginal distributions of $b(\x)$ and is given by $H_B\left( \bn, \bv \right)
=\sum_{j=1}^M \H_j(\b_j) - \sum_{i=1}^N (d_i-1) H_i(b_i)$,
%\begin{align*}
%H_B\left( \bn, \bv \right)
%&=\sum\limits_{j=1}^M \H_j(\b_j) - \sum\limits_{i=1}^N (d_i-1) H_i(b_i), 
%\end{align*}
where $d_i$ is the degree of the variable node $i$ in the factor graph, and $\H_j(\b_j)= -\sum_{y \in S^{N_j}} \b_j(y) \ln \b_j(y)$, $
H_i(b_i)= -\sum_{y \in S} b_i(y) \ln b_i(y)$ denote the entropies of the factor marginal $\b_j(\x_j)$, and the variable marginal $b_i(x_i)$ respectively.
\begin{definition}
Consider a true distribution $p(\x)$ of the form \eqref{eq_factors}. Let $b(\x)$ be a trial distribution. Then, the Bethe free energy $F_B(b)$ is defined as
\begin{align}
F_B(b)&=F_B\left( \bn, \bv \right)=U_B(\bn, \bv) - H_B(\bn, \bv),  \label{eq_bfe_eg}
\end{align}
where $U_B(\bn, \bv)=-\sum_{j=1}^M \sum_{\x_j}  \b(\x_j) \ln f_j(\x_j)$.
\end{definition}

 \subsubsection{Bethe optimization (BO)}
The following optimization problem is referred to as the Bethe optimization.
\begin{align}
&\underset{\bn, \bv} {\arg \min}\; \;  F_B(\bn, \bv), \text{  subject to}  \label{eq_bethe_min}\\
 b_i(x_i) &\geq 0, \hspace{0.4cm} i = 1, \dots, N, \; \;  x_i \in S,\nonumber\\ 
  \sum_{x_i} b_{i} (x_i)&=1, \hspace{0.4cm} i = 1, \dots, N, \nonumber\\ 
\b_j(\x_j) &\geq 0, \hspace{0.4cm} j = 1, \dots, M, \; \;   \x_j \in S^{N_j},\nonumber\\
 \sum_{\x_j} \b_{j} (\x_j)&=1, \hspace{0.4cm} j = 1, \dots, M, \nonumber\\
 \sum_{\x_j \setminus \{x_i \}} \b_j(\x_j)&= b_i(x_i), \hspace{0.2cm} j=1, \dots, M, \; i \in \N_j,\; x_i \in S ,\nonumber
\end{align}
where $\N_j$ is the set of indices of all the variable nodes associated with the factor node $j$.

\emph{Note:}
A feasible collection $(\bn,\bv)$ of the Bethe optimization problem does not necessarily represent the marginals of any coherent joint distribution over $S^N$, and are therefore referred to as \emph{pseudo-marginals} \cite{book_martin}. In spite of performing the optimization over a relaxed set, the solution of the Bethe optimization $(\bn^*, \bv^*)$ exactly coincides with the marginals of the true distribution $(\pn^*, \pv^*)$, if the underlying factor graph is a tree. Further, for factor graphs with loops, the solution leads to very good estimates of the true marginals \cite{book_martin,bethe_emprical}. In fact, in many applications, solving for the global minimizer of \eqref{eq_bethe_min} is not feasible because of its non-convexity. Hence, a stationary point of the BFE satisfying the constraints in \eqref{eq_bethe_min} is considered as a good estimate of the true marginals \cite{book_martin}.


\subsection{Bethe approximation for CSMA}
We observe that the stationary distribution of the CSMA Markov chain $p(\x)$ given by \eqref{eq_succint} is in product from \eqref{eq_factors} with the factor functions $\{f_j \}_{ j=1}^N$ defined as
\begin{align}
f_j(\x_j)= \begin{cases}
\lambda_j, & \text{if }  x_j=1, \gamma_j(\x_j) \geq T, \label{eq_local_factors} \\
  0, & \text{if } x_j=1, \gamma_j(\x_j) < T, \\
 1,  & \text{if } x_j = 0.
\end{cases}
\end{align}
where $\x_j$ is the local schedule of the link $j$ defined earlier.

\begin{comment}
 Using these factor functions, $p(\x)$ can be equivalently represented as
\begin{align}
p(\x)&= \frac{1}{Z}\prod\limits_{j=1}^N f_j(\x_j),  \hspace{0.7cm} \x \in \{0,1\}^\N. \label{eq_dist_prod1}
\end{align}

Next, let us consider the factor graph representation of $p(\x)$. Observe that in $p(\x)$, the number of factor functions are equal to the number of variables nodes $N$, \ie, corresponding to each variable node $j$, there is a factor node $f_j$. For example, if we consider a network with the interference graph (defined in Section \ref{sec_model}) given by Figure \ref{fig_randomgraph}, then the corresponding factor graph is given by Figure \ref{fig_fg_sinr}. 
\end{comment}

By the definition of local feasibility, $p(\x)$ assigns zero probability to a schedule $\x$, if it is locally infeasible at any link. Hence, the factor node marginals $\pn = \{\p_j\}_{j=1}^N$ have to satisfy $\p_j(y)=0, \; \; \; \forall y \notin \I_j, \;  \forall j \in \N.$

\begin{comment}
If we recall the definition of local feasibility, it can be observed that the distribution $p(\x)$ assigns zero probability to a schedule $\x$, if it is locally infeasible at any link $j \in \N$. Hence, the factor node marginals $\pn = \{\p_j\}_{i=1}^N$ have to satisfy  
\begin{align}
\p_j(y)&=0, \; \; \; \forall y \notin \I_j, \;  \forall j \in \N. \label{eq_local_feasibility}
\end{align}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
       \begin{tikzpicture}[scale=0.2]
%\draw (0,0) -- (-2,0.7);
%\draw (-2,-0.7) -- (0,0);
%\draw (1.65,3.65) -- (2.35,3.65);
%\draw (1.65,4.35) -- (2.35,4.35);
%\draw (1.65,3.65) -- (1.65,4.35);
%\draw (2.35,3.65) -- (2.35,4.35);
%\node at (1.0,4) {{$f_{23}$}};
%
%\draw (4-.35,4.5-.35) -- (4+.35,4.5-.35);
%\draw (4-.35,4.5+.35) -- (4+.35,4.5+.35);
%\draw (4-.35,4.5-.35) -- (4-.35,4.5+.35);
%\draw (4+.35,4.5-.35) -- (4+.35,4.5+.35);
%\node at (4,5.5) {{$f_{35}$}};
%
%
%\draw (4-.35,2.5-.35) -- (4+.35,2.5-.35);
%\draw (4-.35,2.5+.35) -- (4+.35,2.5+.35);
%\draw (4-.35,2.5-.35) -- (4-.35,2.5+.35);
%\draw (4+.35,2.5-.35) -- (4+.35,2.5+.35);
%\node at (4,1.5) {{$f_{25}$}};
%
%
%\draw (8-.35,5.5-.35) -- (8+.35,5.5-.35);
%\draw (8-.35,5.5+.35) -- (8+.35,5.5+.35);
%\draw (8-.35,5.5-.35) -- (8-.35,5.5+.35);
%\draw (8+.35,5.5-.35) -- (8+.35,5.5+.35);
%\node at (8,6.5) {{$f_{15}$}};
%
%
%\draw (8-.35,1.5-.35) -- (8+.35,1.5-.35);
%\draw (8-.35,1.5+.35) -- (8+.35,1.5+.35);
%\draw (8-.35,1.5-.35) -- (8-.35,1.5+.35);
%\draw (8+.35,1.5-.35) -- (8+.35,1.5+.35);
%\node at (8,0.5) {{$f_{45}$}};


\draw (2,2)circle(0.4cm);
\node at (1.2,0.9) {{$2$}};
\draw (2,6)circle(0.4cm);
\node at (1.3,7) {{$3$}};
\draw (6,3)circle(0.4cm);
\node at (6.1,4.4) {{$5$}};
\draw (10,8)circle(0.4cm);
\node at (10.7,9) {{$1$}};
\draw (10,-0)circle(0.4cm);
\node at (10.8,-0.7) {{$4$}};
%\node at (3,0.85+0.2) {$2$};



\draw (6+0.2,3-0.2) -- (10-0.2,0+0.35); %3-5
%\draw (10-0.2,0+0.35) -- (8+.35,1.5-.35); %3-5

\draw (10-0.2,8-0.2) -- (6+0.2,3+0.2); %4-3
%\draw (6+0.2,3+0.2) -- (8-.35,5.5-.35); %3-4

\draw (6-0.2,3-0.2) -- (2+0.2,2+0.2); %3-1
%\draw (2+0.2,2+0.2) -- (4-.35,2.5-0); %1-3

\draw (6-0.2,3+0.2) -- (2+0.2,6-0.2); %3-1
%\draw (2+0.2,6-0.2) -- (4-.35,4.5+.35); %1-3

\draw (2,2+0.4) -- (2,6-0.4); %3-1
%\draw (2,6-0.4) -- (2,4+.35); %1-3
\end{tikzpicture}
\caption{interference graph}
\label{fig_randomgraph}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
       \begin{tikzpicture}[scale=0.3]
\draw (-1.5,3)circle(0.4cm);
\node at (-1.5,4) {{$x_2$}};

\draw (0.5,3)circle(0.4cm);
\node at (0.5,4) {{$x_3$}};

\draw (2.5,3)circle(0.4cm);
\node at (2.5,4) {{$x_5$}};
\draw (4.5,3)circle(0.4cm);
\node at (4.5,4) {{$x_1$}};
\draw (6.5,3)circle(0.4cm);
\node at (6.5,4) {{$x_4$}};
%\node at (3,0.85+0.2) {$2$};

\draw (-1.5-.35,0-.35) -- (-1.5+.35,0-.35);
\draw (-1.5-.35,0+.35) -- (-1.5+.35,0+.35);
\draw (-1.5-.35,0-.35) -- (-1.5-.35,0+.35);
\draw (-1.5+.35,0-.35) -- (-1.5+.35,0+.35);
\node at (-1.5,-1) {{$f_{2}$}};

\draw (0.5-.35,0-.35) -- (.5+.35,0-.35);
\draw (0.5-.35,0+.35) -- (.5+.35,0+.35);
\draw (0.5-.35,0-.35) -- (.5-.35,0+.35);
\draw (0.5+.35,0-.35) -- (.5+.35,0+.35);
\node at (.5,-1) {{$f_{3}$}};

\draw (2.5-.35,0-.35) -- (2.5+.35,0-.35);
\draw (2.5-.35,0+.35) -- (2.5+.35,0+.35);
\draw (2.5-.35,0-.35) -- (2.5-.35,0+.35);
\draw (2.5+.35,0-.35) -- (2.5+.35,0+.35);
\node at (2.5,-1) {{$f_{5}$}};

\draw (4.5-.35,0-.35) -- (4.5+.35,0-.35);
\draw (4.5-.35,0+.35) -- (4.5+.35,0+.35);
\draw (4.5-.35,0-.35) -- (4.5-.35,0+.35);
\draw (4.5+.35,0-.35) -- (4.5+.35,0+.35);
\node at (4.5,-1) {{$f_{1}$}};

\draw (6.5-.35,0-.35) -- (6.5+.35,0-.35);
\draw (6.5-.35,0+.35) -- (6.5+.35,0+.35);
\draw (6.5-.35,0-.35) -- (6.5-.35,0+.35);
\draw (6.5+.35,0-.35) -- (6.5+.35,0+.35);
\node at (6.5,-1) {{$f_{4}$}};



\draw (-1.5,0.35) -- (-1.5,3-0.4); %A- x1
\draw (0.5,0.35) -- (0.5,3-0.4); %B- x2
\draw (2.5,0.35) -- (2.5,3-0.4); %B- x2
\draw (4.5,0.35) -- (4.5,3-0.4); %B- x2
\draw (6.5,0.35) -- (6.5,3-0.4); %B- x2

%for node 2
\draw (-1.5,0.35) -- (0.5,3-0.4); %A- x1
\draw (-1.5,0.35) -- (2.5,3-0.4); %A- x1

%for node 2
\draw (0.5,0.35) -- (-1.5,3-0.4); %A- x1
\draw (0.5,0.35) -- (2.5,3-0.4); %A- x1

%for node 5
\draw (2.5,0.35) -- (0.5,3-0.4); %A- x1
\draw (2.5,0.35) -- (-1.5,3-0.4); %A- x1
\draw (2.5,0.35) -- (4.5,3-0.4); %A- x1
\draw (2.5,0.35) -- (6.5,3-0.4); %A- x1

%for node 1
\draw (4.5,0.35) -- (2.5,3-0.4); %A- x1

%for node 4
\draw (6.5,0.35) -- (2.5,3-0.4); %A- x1

\end{tikzpicture}
\caption{Factor graph}
\label{fig_fg_sinr}
    \end{subfigure}
    \caption{Graphs associated with the SINR model}
\end{figure}
\end{comment}
\textbf{BFE for CSMA:}
We shall consider the product form representation of the CSMA stationary distribution $p(\x)$ in \eqref{eq_succint} and compute the BFE. As defined in \eqref{eq_bfe_eg}, the BFE for a given trial distribution $b(\x)$ has two terms $U_B(\bn,\bv)$, $H_B(\bn, \bv)$. The following lemma characterizes the first term $U_B(\bn, \bv)$.
\begin{lemma} \label{lemma_u_bethe}
If the factor marginals of a trial distribution $\bn$, assign zero probabilities to all the infeasible local schedules, \ie, 
 \begin{align}
 \b_j(y)=0, \;  \forall y \notin \I_j, \;  \forall j \in \N, \label{eq_bn_feasible}
 \end{align}
then $U_B(\bn, \bv)$ reduces to $U_B(\bn, \bv)=$ $U_B(\bv)= -\sum_{i=1}^N b_i(1) \ln\lambda_i.$ Moreover, if $\bn$ does not satisfy \eqref{eq_bn_feasible}, $U_B(\bn, \bv)=  \infty$.
\end{lemma}
\begin{proof}
Proof follows from definition of factors in \eqref{eq_local_factors}.
\end{proof}
%\begin{align*}
%U(b)&= -\sum\limits_{\ds \in \{0,1\}^\N} b(\ds) E(\ds), \\
%&=-\sum\limits_{\ds \in \{0,1\}^\N} b(\ds) .\left(-\sum\limits_{a=1}^N \mu_a \left( \ds(\bar{\N_a}) \right)\log(\lambda_a)\right),  \\
%&=-\sum\limits_{a=1}^N \left(\sum\limits_{\dnaa \in \{0,1\}^{\naa}} \mu_a\left( \dnaa \right)b_{\naa}\left(\dnaa\right) \right)\log(\lambda_a),\\
%&= -\sum\limits_{a=1}^N \log(\lambda_a) \E_{b_{\naa}}[\mu_a], \\
%&= -\sum\limits_{a=1}^N \log(\lambda_a) b_a(1).
%\end{align*}

Using Lemma \ref{lemma_u_bethe} and \eqref{eq_bfe_eg}, the BFE for any $(\bn, \bv)$ that satisfies \eqref{eq_bn_feasible} is given by
\begin{align}
F_B(\bn,\bv)&=F_B\left( \{\b_j\}_{j=1}^N,  \{b_i\}_{i=1}^N \right),  \label{eq_bfe}\\
&= \sum\limits_{i=1}^N  -b_i(1) \ln\lambda_i  - \H_i(\b_i)  +  (d_i-1) H_i(b_i), \nonumber
\end{align}
where $d_i$ is degree of variable node $i$ in the factor graph. For $(\bn, \bv)$ that does not satisfy \eqref{eq_bn_feasible}, $F_B(\bn, \bv) = \infty$.


==> subregion_algo.tex <==
\input{figure.tex}
We now propose a distributed algorithm to estimate the fugacities. Each link in the network can independently execute the algorithm once it obtains the a) target service rates of the neighbours, b) the local neighbourhood topology, \ie, which of its neighbours share an edge among themselves in the conflict graph. 


There are mainly two steps in the algorithm at a link $i$. The first step involves computing the maximal cliques\footnote{Note that, this overhead of computing the maximal cliques is involved in the I-GBP algorithm \cite{bp_csma} too.}, and their intersections in which the link $i$ is part of. The next step is to compute its fugacity by using the formula \eqref{eq_main}. We introduce some notations before we present the algorithm.

\emph{Notation:} Let $\Re_0^i$ be the collection of maximal cliques of the conflict graph $G(V,E)$ in which the vertex $i$ is part of. For example, if we consider the graph in Figure \ref{fig_cliq},  then $\Re_0^2 =\{\{1,2\}, \{2,8,7\}$, $\{2,3,7\}\}$. Similarly $\Re_0^3= \{\{2,3,7\}, \{3,5,6,7\}, \{3,4\} \}$. Using the information about the local topology, any standard algorithm like \cite{cliques_complexity} can be used for finding this set of maximal cliques $\Re_0^i$. For every maximal clique $r \in \Re_0^i$, let us associate a constant $c_r=1.$
\noindent\rule[0.5ex]{\linewidth}{0.5pt}
\textbf{Distributed algorithm at link $i$}\\
\noindent\rule[0.5ex]{\linewidth}{0.5pt}
\; \; \emph{Input:}  $\Re_0^i$, service rates $\{s_j\}_{j \in \N_i}$; \hspace{0.25cm}
\emph{Output:}  fugacity $\tilde{v}_i$.
\begin{enumerate}
\item Initialize $l=0$. 

\item Consider the set of all the intersections of the cliques in $\Re_l^i$ to obtain $\Re_{l+1}^i:= \{q_1 \cap q_2 \;|\;  q_1, q_2 \in \Re_{l}^i, q_1 \neq q_2\}.$ If  there are no intersections, \ie, $\Re_{l+1} = \Phi$, go to Step 6; Else continue.

\item From the set $\Re_{l+1}^i$, discard the cliques which are proper subsets of some other cliques in $\Re_{l+1}^{i}$, \ie, discard $r \in \Re_{l+1}^i$ if there exist any other set $q \in \Re_{l+1}^i$ such that $r \subset q$.



\item For each clique $r \in \Re_{l+1}^i$, compute 
\begin{align}
c_r= 1 - \sum_{q \in \S(r)} c_q, \label{eq_counting}
\end{align}
where $\S(r)=\{q \in \cup_{k \leq l}\Re^i_{k}\; | \; r \subset q\}$ is the set of cliques which are super sets of a given set $r$.
\item Increment $l$ by $1$, and go to step 2.

\item Let $\Re^i:= \cup_k \Re_k^i$ denote the collection of all the regions computed above. Then the fugacity is computed as
\begin{align}
\exp(\tilde{v}_i) = s_i \prod_{r \in {\Re^i}} \Big(1- \sum_{j \in r} s_j \Big)^{-c_r}.  \label{eq_main}
\end{align}
\end{enumerate}
\noindent\rule[0.5ex]{\linewidth}{0.5pt}
\emph{Complexity:} The worst case complexity incurred by a link to compute the corresponding maximal cliques $\Re_0^i$ is $O(3^{d/3})$, where $d$ is the the maximum degree of the graph \cite{cliques_complexity}. Hence, for spatial networks, where the degree of the graph does not scale with the network size, our algorithm computes the fugacities with $O(1)$ complexity. 

\emph{Information exchange:} The information exchange required for our algorithm is very limited, since the algorithm is fully distributed except for obtaining the local topology information and neighbours' service rates.

\emph{Simple example:} Let us consider the conflict graph shown in Figure \ref{fig_cliq}, and compute the fugacity for the link $2$ using the proposed algorithm. Then the set of maximal cliques containing the vertex $2$, will be $\Re_0^2 =\{\{1,2\}, \{2,8,7\}$, $\{2,3,7\}\}$. Considering their intersections we get $\Re_1^2=\{\{2,7\}, \{2\}\}$. However, we discard the set $\{2\}$ since it is a proper subset of $\{2,7\}$. Hence $\Re_1^2= \{\{2,7\}\}$. From \eqref{eq_counting}, it can be easily observed that for the set $\{2,7\}$, $c_r=-1$, since it has two super sets namely $q_1=\{2,8,7\}, \;q_2= \{2,3,7\}$  with $c_{q_1}=1, c_{q_2}=1$. As there are no further intersections to be taken in $\Re_1^2$, the following expression gives the fugacity $\exp(\tilde{v}_2)$:
\begin{align*}
\frac{s_2  (1-s_2-s_7)}{(1-s_1-s_2) (1-s_2-s_8-s_7) (1-s_2-s_3-s_7)}.
\end{align*}
Next, we prove that the Region approximated fugacities computed using the clique based approach are exact for a class of graphs called Chordal graphs.
